Effects of Spin-Orbit Coupling and Thermal Expansion on the Phonon-limited Resistivity of Pb from First Principles

Using density functional theory calculations with spin-orbit coupling (SOC), we report on the temperature-dependent thermodynamical properties of Pb: electrical resistivity, thermal expansion (TE), heat capacity, bulk modulus and its pressure derivative. For the former, we employed the state-of-the-art ab initio Boltzmann Transport Equation formalism, and we calculated the effect of TE. In accordance with previous work, we show that SOC improves the description of the phonon dispersion and the resistivity. We argue that this is caused by a joint mutual effect of an increase in the electronic nesting and an increase in the electron-phonon coupling. Interestingly, including TE incorporates non-linearity into the resistivity at high temperatures, whose magnitude depends on whether SOC is included or not. We suggest that mechanisms beyond the quasi-harmonic approximation should be considered to get a better description of Pb with SOC at high temperatures.

==> sections/acknowledgements.tex <==
\begin{acknowledgments}
S. P. acknowledges support from the Fonds de la Recherche Scientifique de Belgique (FRS-FNRS) and the Walloon Region in the strategic axe FRFS-WEL-T.
%
%Computational resources have been provided by the Consortium des Équipements de Calcul Intensif (CÉCI), funded by the FRS-FNRS under Grant No. 2.5020.11 and by the Walloon Region.
This research was financially supported by the Natural Sciences and Engineering Research Council of Canada (NSERC), under the Discovery Grants program Grant No. RGPIN-2016-06666 (M.C.). Computations were made on the supercomputers Beluga and Narval managed by Calcul Québec and the Digital Research Alliance of Canada. The operation of these supercomputers is funded by the Canada Foundation for Innovation, the Ministère de la Science, de l'Économie et de l'Innovation du Québec, and the Fonds de recherche du Québec – Nature et technologies (FRQ-NT). F. A. G. acknowledges the financial support of the FRQ-NT.
\end{acknowledgments}

==> sections/computational_details.tex <==
% Put the figure here to force it on second page
\begin{figure*}[htp!]
    \centering
    \subfloat{\includegraphics{figures/band_structures_combined_with_sliders_v3.pdf}\label{subfig:band_structures_no_lattice_expansion}}
    \subfloat{\label{subfig:band_structures_dos_no_lattice_expansion}}%b
    \subfloat{\label{subfig:band_structures_lattice_expansion_nosoc}}%c
    \subfloat{\label{subfig:band_structures_dos_lattice_expansion_nosoc}}%d
    \subfloat{\label{subfig:band_structures_lattice_expansion_soc}}%e
    \subfloat{\label{subfig:band_structures_dos_lattice_expansion_soc}}%f
    \caption{\label{fig:band_structures}(a) Electronic band structures with (solid orange) and without (dashed blue) SOC computed at the DFT-optimized volume $\Vdft$. (b) The corresponding DOS. (c), (d) Band structure and DOS with varying unit cell volume going from $\delta V/\Vdft=\qtyrange[retain-explicit-plus]{-8}{+12}{\percent}$ without SOC. The shaded area represents where bands from intermediate volumes lie, and the solid curve in the center of the shaded area is for $\delta V/\Vdft=0$. The red shaded area depicts curve with decreasing volume, while the blue shaded area depicts curves of increasing volumes. (e), (f) Same as (c) and (d) with SOC. In all plots, the Fermi level is set at \num{0}. The $\alpha$ and $\beta$ Fermi surface sheets are shown at the bottom of panel (b) in red and blue respectively and are marked with an arrow on panel (a).}
\end{figure*}

\section{Computational Details}
\label{sec:computational_details}

The ground-state properties of Pb were calculated using DFT within a plane wave basis as implemented by the \textsc{Quantum Espresso} (QE) software package~\cite{giannozzi_quantum_2020}. We used an energy cut-off of \qty{90}{\rydberg}, a $(0.5, 0.5, 0.5)$ shifted \numproduct{36x36x36} $\vk$-point mesh and a Gaussian smearing of \qty{1}{\milli\rydberg}. To compute $\Fel$ we use a Fermi-Dirac distribution at the reported temperature. We used DFT within the local density approximation (LDA)~\cite{perdew_self-interaction_1981} and used a fully relativistic ultrasoft~\cite{rappe_optimized_1990} pseudopotential from the PSLibrary version 0.2.2~\cite{dal_corso_pseudopotentials_2014}. The equilibrium volume at \qty{0}{\kelvin}, $\Vdft$, was obtained by optimizing the cell structure until the pressure was less than \qty{0.01}{\kilo\bar}. %Due to the symmetries of fcc Pb, all atomic forces are always exactly 0. 
%With these parameters, the phonon frequencies were converged within \todo{redo phonon smearing convergence} \qty[parse-numbers = false]{X}{\centi\meter^{-1}} at the equilibrium volume. 
The phonon properties were computed using a coarse \numproduct{6x6x6} unshifted $\vq$-mesh from which the phonon dispersion and phonon free energies were obtained using Fourier interpolation. The phonon free energy was computed using frequencies interpolated on a finer \numproduct{64x64x64} $\vq$-mesh in Eq.~\eqref{eq:free_energy_phonons}.
%
Free energy calculations of \cref{eq:free_energy} sampled unit cell volume variations of \qtylist[retain-explicit-plus]{\pm 2;\pm 6;\pm 8;+10;+12}{\percent} around the optimized volume obtained from structural relaxation.
%
The nesting function and phonon linewidth calculations of \cref{eq:nesting_function,eq:phonon_linewidth} were performed on a \numproduct{40x40x40} unshifted $\vk$-mesh and the delta functions were approximated by normalized Gaussian functions with a width of \qty{0.5}{\electronvolt}.
%
The calculations of transport properties (\cref{eq:ibte,eq:relaxation_time,eq:conductivity_tensor}) were carried out using the \textsc{EPW} code~\cite{ponce_epw:_2016,lee_electronphonon_2023} that enables the interpolation of all relevant quantities on fine grids via maximally localized Wannier functions~\cite{giustino_electron-phonon_2007,marzari_maximally_1997,souza_maximally_2001,pizzi_wannier90_2020}. Thus, the phonon frequencies $\omega_{\vq\nu}$, electronic eigenvalues $\epsilon_{n\vk}$, electron velocities $\vv_{n\vk}$ and EPC matrix elements $g_{mn\nu}(\vk,\vq)$ were computed on a \numproduct{60x60x60} $\vk$ and $\vq$ meshes. To speed up fine-grid interpolation, the coarse \numproduct{36x36x36} $\vk$ grid used to compute the SCF ground state was downsampled using a non-SCF calculation to an unshifted \numproduct{12x12x12} $\vk$-grid. Extensive convergence studies with respect to to carse and fine momentum grid sizes are given in the Supporting Information (SI)~\cite{Goudreault2024_SI}. Finally, the computation of \cref{eq:ibte,eq:relaxation_time} requires the evaluation of Dirac delta distributions, which are approximated using state-dependent Gaussian adaptive broadening approach detailed in Refs.~\cite{ponce_first-principles_2021_hall} and~\cite{li_shengbte_2014} which is implemented in \textsc{EPW} to avoid convergence studies with respect to this parameter.

==> sections/conclusion.tex <==
\section{Conclusion}

We computed the thermodynamical properties of Pb and assessed the impact of SOC. % We relied on a third-order Birch-Murnaghan EOS fit of the total volume and temperature-dependent free energy computed within the QHA and where we included the entropic effect due to thermal electronic excitations via Mermin's approach. We observed that the latter is completely negligible compared to the phonon part of the free energy. 
% From the fit, we extracted the temperature-dependent bulk modulus, its pressure derivative, and lattice parameter. 
In all cases, we obtained relatively good agreement with experiments, especially for the TE where SOC agrees with the experimental values closely. As for the phonon frequencies, where a strong softening is observed with SOC, the bulk modulus and its pressure derivative all undergo a similar decrease. Only the heat capacity displayed a better agreement with experiments without SOC than with it. To shed light on these results, we computed the electronic nesting function, the phonon linewidth $\gamma_{\vq\nu}$ and a $g$-weighted nesting function $\gamma_{\vq\nu}/\omega_{\vq\nu}$. We showed that the nesting function might not be sufficient to explain the phonon softening, especially at $\vq=X$ where it is the largest. We argued that it is induced by a combined effect of the EPC matrix elements being increased by the softening itself, which, in turn, would increase the softening until self-consistency is achieved. In the end, the difference with SOC is mostly seen in the EPC matrix elements, which is stronger with SOC than without, especially at $X$, where the nesting function peaks.

% We showed that the nesting was indeed globally higher with SOC than without it, despite SOC having close to no effect on the electronic structure. Nonetheless, the nesting peaks at $\vq=X$ both with and without SOC, suggesting that nesting is not sufficient to explain the strong phonon softening at this point. Adding EPC matrix elements to take into account transition probabilities showed a strong enhancement of the nesting at $X$ with SOC than without where it remains much smoother. As such, this suggests that the phonon softening and the EPC mutually influence each other, so that the final effect is a net phonon softening when SOC is turned on. Finally, as the phonon softening with SOC is strongly enhanced when changing the volume, we showed that the volumetric dependence of the EPC matrix element is almost entirely contained within the frequencies as the phonon linewidth are pretty much volume-independent compared to the electronic nesting function and its $g$-weighted version analog.

We then computed the phonon-limited temperature-dependent resistivity of Pb from first principles using the state-of-the-art IBTE formalism both with and without SOC. We obtained results similar to previously reported resistivity data obtained via the LOVA approach, where the best agreement with experiments was obtained with SOC. Thus, we note that the IBTE approach does not yield a significant difference from the LOVA in the particular case of Pb. In an attempt to improve results at high temperatures, we incorporated the TE effects by using the temperature-dependent lattice parameter obtained by minimizing the free energy. With TE, non-linearity did appear at high temperature, but the computed resistivity is subject to a large increase with SOC as compared to that without SOC resulting in an overestimation with respect to experiments. To understand these results, we investigated the scattering rate and noticed that TE had a similar effect than SOC, while including both makes the inverse relaxation times double, which explains the resistivity behavior with these parameters. This non-linear effect with expanding volume correlates with the volume dependency of the $\gamma_{\vq\nu}/\omega_{\vq\nu}$ function, hinting that the strong phonon softening caused by lattice expansion transfers to the relaxation times and the resistivity.

Among possible avenues to improve this behavior at high temperature, one could include the choice of exchange-correlation functional (XC) as it generally have strong effects on the phonon properties, especially in \ce{Pb}~\cite{grabowski_ab_2007,verstraete_density_2008}. A comparative study of the thermodynamical properties of \ce{Pb} without SOC was already carried out by \citet{grabowski_ab_2007} where the authors compared the LDA and PBE XC. As such, since all our results were obtained with the LDA, further investigations should compare the effects of the XC on the resistivity while considering TE and SOC. Other XC functionals such as the recently developed r\textsuperscript{2}SCAN~\cite{furness_accurate_2020} could also be interesting to investigate, however for the latter, its implementation in DFPT frameworks has yet to be done. Alternatively, one could investigate mechanisms beyond the QHA such as temperature dependent effective potentials (TDEP)~\cite{knoop_tdep_2024} or the stochastic self-consistent harmonic approximation~\cite{monacelli_pressure_2018,bianco_second-order_2017,errea_anharmonic_2014,errea_first-principles_2013} in order to improve the overly softened phonon dispersions seen in this work. Additionally, considering the phonon self-energy and including non-anharmonic contributions could also improve the phonon dispersions as demonstrated in \ce{PbTe} where a strong renormalization was observed at high temperature~\cite{romero_thermal_2015}.

==> sections/discarded/OLDmethod.tex <==
\section{Method}

\begin{itemize}
    \item Use DFT and DFPT as implemented in the Quantum Espresso\cite{giannozzi_quantum_2020} software to get physical properties on coarse grids.
    \item Interpolation on very fine grids using maximally localized wannier functions for both electronic structure\cite{marzari_maximally_1997,souza_maximally_2001} and phonon properties\cite{giustino_electron-phonon_2007} using the EPW code\cite{ponce_epw:_2016}. Using EPW we then compute the conductivity of materials by solving iteratively the BTE.
\end{itemize}

\section{Computational Details}

All calculations were done using the \textsc{Quantum Espresso} software package suite\cite{giannozzi_quantum_2020}. 

\subsection{Pb}
Ground state Kohn-Sham energies were obtained by using a plane-wave basis with an energy cutoff of 90 Rydbergs on a $36\times 36\times 36~\vk$-point grid in the full first BZ yielding 4218 irreducible $\vk$-points. A Gaussian smearing was used with a spread of $10^{-3}$ Rydbergs. We used The ground state total energy was converged up to $10^{-16}$ Rydbergs in order to get accurate phonon frequencies. Phonon dispersions were well converged with a $6\times 6\times 6~\vq$-point grid in the full first BZ yielding 16 irreducible $\vq$-points. The potential derivatives were converged within $10^{-16}$ Rydbergs as well to ensure accuracy of the phonon frequencies.

==> sections/discarded/method_theory.tex <==
\section{Method}
\label{sec:method}
\todo{This is probably too detailed, we'll cut stuff later.}
%In all the following, we employ the rigid band approximations which implies that the band structure remains unchanged under electronic excitations or other perturbations like an electric field. 
To compute the transport properties of Pb, we make use of the linearized Boltzmann Transport Equation with electron-phonon interactions as the only diffusive process. In this formalism, the conductivity is defined as \cite{ponce_towards_2018,ziman_electrons_1960,li_electrical_2015,ponce_first-principles_2020}:

\begin{equation}
    \label{eq:conductivities}
    \sigma_{\alpha\beta} = \sum_n\int\frac{d^3\vk}{(2\pi)^3}v_{n\vk,\alpha}\partial_{E_\beta}f_{n\vk},
\end{equation}

where $\partial_{E_\beta}f_{n\vk}$ is the derivative of the occupation function for the Kohn-Sham state in band $n$ and wavevector $\vk$ labeled $\ket{n\vk}$ with respect to an applied electric field $\boldsymbol{E}$ evaluated at $\vE=0$ and $\vv_{n\vk,\alpha}$ is the diagonal group velocity matrix element in the $\alpha$ direction which is defined as\cite{starace_length_1971,ponce_epw:_2016}:

\begin{equation}
    \label{eq:group_velocity}
    \vv_{n\vk,\alpha}=\braket{n\vk|i[\mathcal{H}, \vecr_\alpha]|n\vk},
\end{equation}

with $\mathcal{H}$ being the system Hamiltonian and $\vecr_\alpha$ the $\alpha$ component of the position operator. In a sense, Eq. \eqref{eq:conductivities} is an average of all electronic velocities whose occupation changes under an electric field. Eq. \ref{eq:group_velocity} includes the effect of the non-local part of the DFT potential which have been taken into account in this work. In the context of electron-phonon interactions and phonon-limited diffusion, the BTE can be linearized and the $\partial_{E_\beta}f_{n\vk}$ can be obtained by solving the implicit equation\cite{ponce_towards_2018,ponce_first-principles_2020,li_electrical_2015}:

\begin{align}
    \label{eq:bte_occupations}
    \nonumber
    &\partial_{E_\beta}f_{n\vk} = ev_{n\vk,\beta}\tau_{n\vk}\frac{\partial f^0_{n\vk}}{\partial\epsilon_{n\vk}} + \frac{2\pi\tau_{n\vk}}{\hbar}\sum_{m\nu\sigma}\int\frac{d^3\vq}{\OmegaBZ}|g_{mn\nu}^{\vk,\vq}|^2\\
    &\times[(1+\sigma)/2-\sigma f^0_{n\vk}+n_{\nu\vq}]\delta(\Delta_{\vk\vq}^{nm}+\sigma\hbar\omega_{\vq\nu})\partial_{E_\beta}f_{m\vk+\vq},
\end{align}

where $g_{mn\nu}^{\vk,\vq}=\braket{m\vk+\vq|\partial_{\nu\vq}V^{SCF}|n\vk}$ is the electron-phonon matrix elements whose squared amplitude is interpreted as the probability of an electron to scatter from state $\ket{n\vk}$ to state $\ket{m\vk+\vq}$ via the emission or absorption of a phonon with branch index $\nu$ and wavevector $\vq$, $e$ is the electron charge, $n_{\vq\nu}$ is the Bose-Einstein distribution evaluated at energy $\hbar\omega_{\vq\nu}$, $\sigma\in\{+1,-1\}$ stands for phonon absorption/emission processes, $\Delta_{\vk,\vq}^{nm} = \epsilon_{n\vk}-\epsilon_{m\vk+\vq}$ and $\OmegaBZ$ is the Brillouin Zone volume. Finally, $f^0_{n\vk}=\left[\exp((\epsilon_{n\vk}-\mu)/k_BT)+1\right]^{-1}$ is the unperturbed electronic occupation function for state $\ket{n\vk}$ corresponding to the Fermi-Dirac distribution with $k_B$ the Boltzmann constant and $\mu$ the chemical potential. We note that truncating Eq. \eqref{eq:bte_occupations} at it's first term is called the Self-Energy Relaxation Time Approximation (SERTA). $\tau_{n\vk}$ is the electron-phonon relaxation time which can be derived from Fermi's golden rule and is written as\cite{grimvall1981electron}:

\begin{align}
    \label{eq:relaxation_time}
    \nonumber
    &\tau_{n\vk}^{-1} = \frac{2\pi}{\hbar}\sum_{m\nu\sigma}\int\frac{d^3\vq}{\OmegaBZ}|g_{mn\nu}^{\vk,\vq}|^2\\
    &\times[(1+\sigma)/2 -\sigma f^0_{m\vk+\vq}+n_{\vq\nu}]\delta(\Delta_{\vk,\vq}^{nm}-\sigma\hbar\omega_{\vq\nu})
\end{align}

In Eq. \eqref{eq:conductivities}, \eqref{eq:bte_occupations} and \eqref{eq:relaxation_time}, $\alpha$ and $\beta$ indices denote cartesian coordinates. In these equations, temperature effects are only included through the chemical potential $\mu$ and occupation functions $f^0_{n\vk}$ and $n_{\vq\nu}$. In order to take into account thermal lattice expansion effects, we compute all these equations separately for each lattice parameters at the given temperature which increases the computational cost significantly.

%Within Boltzmann's transport theory, the electrical current density is a simple average of fermi velocities:

%\begin{equation}
%    \label{eq:current_density}
%    J_i = \sum_n\int\frac{d^3\boldsymbol{k}}{(2\pi)^3}v^i_{n\vk}f_{n\vk},
%\end{equation}

%where $J_i$ is the current density component along direction $i\in{x, y, z}$, $n$ is a band index, $\vk$ is a reciprocal vector, $v^i_{n\vk}=\nabla_{\vk}\epsilon_{n\vk}$\todo{commutateur avec potentiel non-local?} is the velocity matrix element, $\epsilon_{n\vk}$ is the electronic dispersion, $f_{n\vk}$ is the occupation number and the integral is carried out on the first Brillouin zone while the sum runs over all bands. Differientiating 

The temperature-dependent lattice parameter $a(T)=\sqrt[3]{V}$ of Pb was computed by minimizing the Helmoltz free energy $F(V, T)$ of the system with respect to the unit cell volume $V$ at each temperature $T$. In crystals, this free energy can be decomposed in an electronic-only term $F_{\text{el}}$ and one due to phonons $F_{\text{ph}}$:

\begin{equation}
    \label{eq:free_energy}
    F(V,T)=F_{\text{ph}}(V,T) + F_{\text{el}}(V,T).
\end{equation}

Within the Quasi-harmonic approximation (QHA), the vibrationnal term can be written as\cite{baroni_density-functional_2010,palumbo_lattice_2017}

\begin{align}
    \label{eq:free_energy_phonons}
    \nonumber
    F_{\text{ph}}(V,T)=&\frac{1}{2N}\sum_{\vq\nu}\bigg\{\hbar\omega_{\vq\nu}(V)\\
    &+kT\ln\left.\left[1-\exp\left(-\frac{\hbar\omega_{\vq\nu}(V)}{kT}\right)\right]\right\},
\end{align} 

where $N$ is the number of cell in the material and $\omega_{\vq\nu}(V)$ is the phonon frequency for branch $\nu$ and wavevector $\vq$ for a given primitive cell volume $V$. Meanwhile, $F_{\text{el}}(V,T)$ is the electronic contribution to the free energy and is written as\cite{mermin_thermal_1965}

\begin{equation}
    \label{eq:free_energy_electrons}
    F_{\text{el}}(V,T)=U_{\text{el}}(V,T) - TS_{\text{el}}(T,V),
\end{equation}

where $U_{\text{el}}$ is the electronic internal energy at finite temperature for a unit cell volume $V$ and the entropy $S_{\text{el}}(T,V)$ is computed as

\begin{equation}
    \label{eq:entropy}
    S_{\text{el}}(T,V) = -\sum_{i}f_i\ln f_i + (1-f_i)\ln(1-f_i),
\end{equation}

where $i$ is a composite index running over spins, $\vk$ and band and $f_i=f_i(T,V)$ is the occupation factor for an electron in state $i$. In order to minimize Eq. \ref{eq:free_energy} at various $T$, we compute all quantities using DFT at various volumes and temperatures. Then, we fit $F(V, T)$ at each sampled temperature with the third-order Birch-Murnaghan isothermal equation of state defined as\todo{add Birch murnghan source}

\begin{align}
    \begin{split}
        F(V, T) = E_0 +& \frac{9B_0V_0}{16}\left[\left(\frac{V_0}{V}\right)^{\frac{2}{3}}-1\right]^2\\
        &\times\left\{\left[\left(\frac{V_0}{V}\right)^{\frac{2}{3}}-1\right]B_0' + \left[6-4\left(\frac{V_0}{V}\right)^{\frac{2}{3}}\right]\right\},
    \end{split}
\end{align}

where $V_0$ is the equilibrium volume, $E_0$ is the minimum of energy at $V_0$, $B_0$ is the bulk modulus at $V_0$ and $B_0'$ is the derivative of the bulk modulus w.r.t. pressure at $V_0$. Extracting $V_0$ from the fit at each sampled temperature yields the temperature-dependant lattice parameter $a(T)=\sqrt[3]{V_0(T)}$.\\

In non-metallic materials, the temperature dependence of the electronic contribution to the total free energy $F_{\text{el}}$ can safely be ignored if the electronic gap is much larger than thermal energies\cite{ponce_hole_2019}. However, in metals, this is not the case and one cannot justify this approximation. Various methods exist in order to compute this temperature dependence and a previous work quantified the errors made by these different approaches in transition elements\cite{zhang_accurate_2017}. In this work, we used to most accurate method which is Mermin's approach\cite{mermin_thermal_1965}.

% where $U_{\text{el}}(V,T)$ and $S_{\text{el}}(T,V)$ are written as:

% \begin{equation}
%     \label{eq:Uel}
%     U_{\text{el}}(T,V) = \int_{-\infty}^\infty E\cdot\text{DOS}(E)f^0 dE - \int_{-\infty}^{E_F}E\cdot\text{DOS}(E)dE
% \end{equation}

% and

% \begin{equation}
%     \label{eq:Sel}
%     S_{\text{el}}(T,V)=-k\int_{-\infty}^\infty[f^0\ln f^0 + (1-f^0)\ln(1-f^0)]\text{DOS}(E)dE,
% \end{equation}

% where $E_F$ is the fermi level, $\text{DOS}(E)$ is the density of states and $f^0=f^0(\mu,T,E)$ is the Fermi-Dirac distribution at energy $E$ and temperature $T$ for chemical potential $\mu$. The chemical potential can be computed from the constraint of the number of electrons per cell $N_{\text{el}}$:

% \begin{equation}
%     \label{eq:chemical_potential}
%     N_{\text{el}} = \int_{-\infty}^\infty\text{DOS}(E)f^0dE.
% \end{equation}

==> sections/discarded/results.tex <==
\section{Results}
% \begin{itemize}
%     \item Pb properties: FCC with 1 atom in the unit cell. Lattice parameters, 
%     \item phonon dispersion + discuss kohn anomaly with kgrid convergence of phonon dispersion\cite{corso_ab_2008,heid_effect_2010}. SOC seems important to describe accurately the phonon dispersion and electron-phonon coupling. Phonon dispersion exp data from Brockhouse\cite{brockhouse_crystal_1962}.
%     \item Discuss SERTA vs fully self consistent resistivity curves?
%     \item Discuss effects of SOC vs no SOC
%     \item Discuss effects of lattice constants and consider lattice parameters expansions. Exp data for lattice parameter expansion comes from\cite{feder_use_1958}. Partial conclusion: lattice parameters gives important effects on resistivity calculation (why? perhaps it changes a lot the electron phonon matrix elements / frequencies / electronic dispersions).
%     \item Discuss IBTE vs Ziman. Experimental resistivity measurements come from\cite{moore_absolute_1973,leadbetter_energy_1966,cook_thermal_1974,hellwege_electrical_1982}
% \end{itemize}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/Pb/final_ph_disp_comparison.pdf}
    \caption{Phonon dispersion of Pb computed with a LDA XC functional. Dashed curve includes SOC while plain curves do not. Colors differentiate between different lattice parameters: $a_{\text{SOC}}$ (blue) stands for the optimized lattice parameter with SOC, $a_{noSOC}$ (orange) is the optimized lattice parameter without SOC and $a_{exp}$ is the experimental one (green). White dots are inelastic neutron scattering data taken from \cite{brockhouse_crystal_1962} ($T=100K$).}
    \label{fig:pb_phonon_dispersion}
\end{figure}


Figure \ref{fig:pb_phonon_dispersion} compares the phonon dispersion of lead with respect to the lattice parameter (different colors). The lattice parameters used are listed on table \ref{tab:pb_lattice_parameters} where the relaxed parameters were obtained by converging the primitive cell pressure within $5\times 10^{-3}$ kbar. For each of these, we compare the dispersions with (dashed) and without (plain) SOC. 
%For instance, the orange dashed curve of figure \ref{fig:pb_phonon_dispersion} represents the phonon dispersion computed with SOC but using the lattice parameter relaxed without SOC, etc.
As reported by several other work\cite{heid_effect_2010,verstraete_density_2008,corso_ab_2008,liu_linear-response_1996}, we see that SOC is important in order to get phonon frequencies closer to experiments. Indeed, for a given lattice parameter, including SOC (going from a plain curve to a dashed one in Fig. \ref{fig:pb_phonon_dispersion}) softens the phonon modes. Indeed, SOC typically yields a higher nesting which, in turn, softens the phonon modes\todo{cite where this comes from: my source = Michel for now}. We see also that the phonon softening is maximal near the $X$ and $L$ points. Additionally, the lattice parameter in itself also bears a strong influence on the phonon dispersion as can be seen by the green curve which is the phonon frequencies with the experimental lattice parameter. This is also expected as increasing the lattice spacing decreases the ionic potential between atoms which, in turn, softens the phonon frequencies. As seen from Fig. \ref{fig:pb_phonon_dispersion}, the most accurate dispersion w.r.t. inelastic neutron diffraction data is computed from an optimized lattice parameter with SOC. Previous work by Rittweger \etal, did not include SOC but rather used the experimental lattice parameter\cite{rittweger_phonon_2017}. Even though SOC is important, they obtained relatively good phonon dispersions

Indeed, a higher lattice parameter makes the interatomic bonds weaker which yields lower phonon frequencies. This effect can be seen on figure \ref{fig:pb_phonon_dispersion} where a higher lattice parameter lowers

%One of the very first fully ab initio calculation of Pb's resistivity was carried out by Savrasov et al. in 1996 \cite{savrasov_electron-phonon_1996}. This attempt was done in the early beginnings of electron-phonon calculations with DFPT and the LOVA approach (also called the Ziman's resistivity formula) was used to get the resistivity from the Eliashberg function. Although a good agreement with experiments was obtained in general in Pb and other simple metals like Al, Pd, Cu, etc., a discrepency could still be found at high temperature which could be explained by many factors. For example, the inaccuracy of the LOVA approach can be easily argued since that formula was developped assuming a single spherical and isotropic Fermi surface\cite{ziman_electrons_1960}, which is completely inaccurate in Pb where there is two distinct non-spherical and highly distorted Fermi sheets\cite{bertoni_third_1974,anderson_fermi_1965}. More recently, a detailed study of the phonon limited transport scattering rates as computed from the IBTE formalism has been conducted by Rittweger et al.\cite{rittweger_phonon_2017}. As mentioned in section \ref{sec:theory}, the IBTE is a more general method than the LOVA approach where no assumption on the Fermi surface is made prior to the resistivity calculation.\\

% \subsection{Effects of Spin-Orbit Coupling}
%Interestingly enough, both these studies didn't include relativistic and SOC effects. Indeed, as pointed out by several authors \cite{vosko_influence_1965,corso_ab_2008,anderson_fermi_1965}, since Pb is a heavy element ($Z=82$), an accurate treatment of this material should include them. They can indeed have a strong influence on lattice dynamics and consequentely, on the phonon-limited resistivity, the phonon frequencies and the electron-phonon coupling matrix elements.% For example, the figure \ref{fig:pb_phonon_dispersion} shows the computed phonon dispersion of Pb with and without SOC compared to experimental values taken from inelastic neutron scattering data\cite{brockhouse_crystal_1962,woods1961inelastic}. As one can see, the dispersion with SOC agrees more with experiments than the one without SOC which is consistent with results from previous studies\cite{ponce_epw:_2016,corso_ab_2008}.\\
%The curves were computed on a $6\times 6\times 6$ $\vq$-point grid from a ground state calculation computed on a shifted $14\times 14\times 14$ $\vk$-point grid with a gaussian smearing of 0.025Ry and an energy cutoff of 90Ry. A fully relativistic LDA pseudopotential was used throughout all Pb calculations. The relaxed lattice parameters of $a=9.322$ bohr without SOC and $a=9.258$ bohr with SOC. 
% the calculation parameters
% The dispersion curves were interpolated from a fully consistent DFPT calculation carried on a $6\times 6\times 6$ $\vq$-point grid. Calculations without SOC were drawn from a ground state calculation done on a $12\times 12\times 12$ $\vk$-point grid while the ones with SOC were done on a much denser grid of $24\times 24\times 24$ $\vk$-point grid. It was indeed noticed that, in order to achieve convergence for all phonon wavevectors ($\vq$-points), especially at $X$ in the first Brillouin Zone (FBZ), the ground state required a denser $\vk$-point grid when employing SOC. Otherwise, a strong phonon softening was observed for this $\vq$-point in particular. For all calculations, the lattice parameters used were $a_0=4.874\AA$ without SOC and $a_0=4.899$ with SOC which are the relaxed lattice parameters for this setup. A norm-conserving pseudopotential was used with an energy cutoff of 90Ry and an artificial temperature smearing of 1mRy.

% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{figures/Pb/phonon_dispersion_vs_exp.pdf}
%     \caption{Phonon dispersion of Pb with (dashed line) and without (plain line) SOC compared to experimental values taken from ref \cite{brockhouse_crystal_1962,woods1961inelastic}.}
%     \label{fig:pb_phonon_dispersion}
% \end{figure}


\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/Pb/all_ibte_curves_with_exp.pdf}
    \caption{Resistivity of Pb as computed with the IBTE scheme compared with the experimental values (black dots)\cite{moore_absolute_1973,leadbetter_energy_1966,cook_thermal_1974,hellwege_electrical_1982}. The figure shows results including SOC (dashed) and without SOC (plain) and different lattice parameter treatments: using experimental lattice parameter at room temperature (red), relaxed lattice parameter at $T=0K$ (blue), experimental lattice parameters including thermal lattice expansion (green) and thermal lattice expansion as computed from the equation of state fit (yellow).}
    \label{fig:Pb_IBTE}
\end{figure}

% \subsection{Effects of Thermal Lattice Expansion}

Another important effect which might affect the lattice dynamics is the lattice size. Indeed, increasing the lattice parameters yields a lower interatomic force constant which translates into lower phonon frequencies and EPC matrix elements. When studying the resistivity of materials with respect to the temperature, one might need to consider these effects as well. %From a perspective of fully ab-initio calculations, 
The phonon-limited resistivity depends on the phonon frequencies thus making their computation critical to get an accurate result. These frequencies are, in turn, highly dependend on different DFT parameters such as the $\vk$-point sampling or the XC functional, but they also depend on physical parameters such as the atomic masses and the lattice spacing. Indeed, a lower lattice spacing would decrease the distance between atoms which would increase the interatomic force constants which, in turn, would increase the phonon frequencies. Since real materials are subject to thermal expansion effects, these could ultimately induce changes in the phonon-limited resistivity. These effects are not taken into account by plain DFT calculations. To do so, we need to consider the total free energy of the system at a given temperature $T$ and unit cell volume $V$:
\begin{align}
    \label{eq:total_free_energy}
    \begin{split}
        F(V, T) &= E^{KS}(V) + F_0(V) + F_{\text{thermal}}(V, T),\\
        F_0(V) &= \frac{1}{2}\sum_{\vq\nu}\hbar\omega_{\vq\nu}(V),\\
        F_{\text{thermal}}(V,T) &= k_BT\sum_{\vq\nu}\ln\left(1-\exp\left\{-\hbar\omega_{\vq\nu}(V)/k_BT\right\}\right),
    \end{split}
\end{align}
where $\omega_{\vq\nu}$ is the phonon frequencies at wavevector $\vq$ and for branch $\nu$, $E^{KS}(V)$ is the total DFT energy which depends on the volume $V$, $F_0(V)$ corresponds to the zero point energy and $F_{\text{thermal}}(V,T)$ accounts for the thermal free energy which comes from the phonon partition function[CITER LE LIVRE A VERO?]. To get the thermal lattice expansion from equation \eqref{eq:total_free_energy}, we need to fit it to an equation of state that relates the volume dependent free energy $F(V, T)$ to the equilibrium volume $V_0(T)$ at a given temperature or pressure like the Birch-Murnaghan equation of state:

\begin{align}
    \begin{split}
        F(V, T) = E_0 +& \frac{9B_0V_0}{16}\left[\left(\frac{V_0}{V}\right)^{\frac{2}{3}}-1\right]^2\\
        &\times\left\{\left[\left(\frac{V_0}{V}\right)^{\frac{2}{3}}-1\right]B_0' + \left[6-4\left(\frac{V_0}{V}\right)^{\frac{2}{3}}\right]\right\},
    \end{split}
\end{align}

where $E_0$ the free energy at the equilibrium volume, $B_0$ is the bulk modulus at the equilibrium volume and $B_0'$ the derivative of the bulk modulus at the equilibrium volume. Figure \ref{fig:Pb_lattice_expansion} shows the lattice parameters $a(T)=\sqrt[3]{V_0(T)}$ in function of $T$ obtained via this fitting procedure compared to the experimental measurements taken from ref\cite{feder_use_1958}. The inset shows the relative variation of $a(T)$ compared to the one at room temperature ($a_0$). One can see first that DFT can capture a sense of thermal lattice expansion but does not seem to fit well the experiments. This was expected as it is well known that, depending on the XC functional, DFT usually under/over-estimate (LDA/PBE) the lattice parameters due to an under/over-estimation of the charge screening effects. Nonetheless, regardless of the XC functional used, the relative variation of the lattice parameter compared to the one at room temperature ($\delta a/a_0$) seems to follow quite well the experimental data (see insert of figure \ref{fig:Pb_lattice_expansion}) which seems promising. However, when we add SOC effects, the lattice parameters increase drastically as well as it's derivative. Also, at high temperature, it seems that the lattice expansion is not linear. This might be a spurious effect coming from negative phonons at high volume. Indeed, when including SOC, the phonon frequencies near $\vq=X$ seems to undergo a strong softening when the volume is increasing. This effect does not occur without SOC. We tried computing the phonon frequencies using denser $\vk$-grids and higher smearing to see if it was a convergence issue but the softening occured more rapidly in this case, suggesting that a strong nesting is happening.


One can see that DFT calculations are able to capture very well the relative variation of the lattice parameters with respect to their values at room temperature although the absolute value of the lattice parameter strongly depends of the XC functional that was used. Oddly, when taking into account the SOC effects, the variation of the lattice parameters seems to be much higher than excluding it even though including SOC upgrades the DFT calculation to a higher level of theory making it, in principle, more physically accurate, especially for Pb. This discrepancy carries through the whole workflow up to the IBTE calculation where we can see that including SOC brings a lot of non-linarity into the resistivity compared to the case without it. This is seen on figure \ref{fig:Pb_IBTE} where the dashed yellow curve diverges quite fast from the experimental values compared with the other calculations.

\begin{figure}
    \centering
    %includegraphics[width=\columnwidth]{figures/Pb/lattice_expansion_final_variation_prettier.pdf}
    \includegraphics[width=\columnwidth]{figures/Pb/lattice_expansion_combined.pdf.png}
    \caption{The relative variation of the lattice parameter of Pb versus the one at room temperature in function of temperature. Comparison between the DFT predicted curves and experimental values from Ref. \cite{feder_use_1958}. Comparison of the effects of SOC (dashed) and without it (plain) and comparing the effects of different exchange-correlation functionals: LDA (red) and PBEsol (blue).}
    \label{fig:Pb_lattice_expansion}
\end{figure}



==> sections/ground_state_properties.tex <==

\subsection{Ground State and Volumetric Effects}
\label{sec:equilibrium_properties}

\begin{figure*}[htp!]
    \centering
    % \includegraphics{figures/phonon_dispersions_combined_with_sliders.pdf}
    \subfloat{\includegraphics{figures/phonon_dispersions_combined_with_sliders_v3.pdf}\label{subfig:phonon_dispersions_no_lattice_expansion}}
    \subfloat{\label{subfig:phonon_dispersions_lattice_expansion_nosoc}}%b
    \subfloat{\label{subfig:phonon_dispersions_lattice_expansion_soc}}%c
    \caption{\label{fig:phonon_dispersions}(a) Phonon dispersion of Pb with (dashed orange) and without (plain blue) SOC computed at the DFT-optimized lattice parameter. Black circles are neutron diffraction experimental data at \qty{100}{\kelvin} from Ref.~\cite{brockhouse_crystal_1962} ($\times$ markers) and from Ref.~\cite{brockhouse_old_1961} (open and closed circles). (b) Phonon dispersion of Pb without SOC at different volumes. The relative volume difference $\delta V/\Vdft$ is denoted by the curve color where red corresponds to $\delta V/\Vdft =\qty{-8}{\percent}$ and magenta to $\delta V/\Vdft =\qty[retain-explicit-plus]{+12}{\percent}$. (c) Same as (b) with SOC.}
\end{figure*}

%Tab. \ref{tab:pb_lattice_parameters} shows the resulting optimized lattice parameters $a$ compared to the experimental value at room temperature.
The relaxed geometry yielded a lattice parameter of \qty{4.881}{\angstrom} without SOC and \qty{4.882}{\angstrom} with SOC. These values are within \qty{0.5}{\percent} of the experimental lattice parameter extrapolated at $T\rightarrow \qty{0}{\kelvin}$ which is \qty{4.905}{\angstrom}\cite{grabowski_ab_2007}.
% \todo{is this table really necessary? we could just list obtained values in the text.}
% \setlength\tabcolsep{0pt}
% \begin{table}[h!]
%     \centering
%     \begin{tabular*}{\columnwidth}{@{\extracolsep{\fill}} llll}
%         \hline\hline
%         SOC & XC & $a$ [\AA] & Reference\\
%         \hline
%         \multirow{5}{*}{No} & PBE & 5.043 & \cite{grabowski_ab_2007}\\
%         & LDA & 4.884 & \cite{grabowski_ab_2007}\\
%         & LDA & 4.884 & \cite{corso_ab_2008} \\
%         & LDA & 4.880 & \cite{ponce_epw:_2016}\\
%         & LDA & 4.881 & this work\\
%         & & &\\
%         \multirow{3}{*}{Yes} & LDA & 4.882& this work\\
%             & LDA & 4.884 & \cite{corso_ab_2008}\\
%             & LDA & 4.905 & \cite{ponce_epw:_2016}\\
%         & & &\\
%         & Exp. ($T\rightarrow 0$ K) & 4.905 & \cite{grabowski_ab_2007}\\
%          \hline\hline
%      \end{tabular*}
%      \caption{Optimized lattice parameter $a$ of Pb as computed from DFT for different exchange-correlation functionals (XC) compared to the experimental value extrapolated to $0$ K.}
%      \label{tab:pb_lattice_parameters}
% \end{table}
Consistent with previous reports~\cite{heid_effect_2010,corso_ab_2008,verstraete_density_2008}, SOC only changes the optimized lattice parameter by \qty{0.02}{\percent}. %It is known that the optimized geometry obtained using this LDA exchange-correlation (XC) functional underestimates the lattice parameter compared to experimental data. One could use another % , more computationally expansive 
% XC like the PBE/GGA~\cite{perdew_generalized_1996} in order to get an optimized lattice parameter closer to the experiment. As reported by Refs.~\cite{grabowski_ab_2007,verstraete_density_2008}, using PBE/GGA does indeed yield a larger lattice parameter value in Pb. However, this increased lattice parameter also results in softer phonon frequencies, which is an indirect consequence of such an XC~\cite{skelton_influence_2015,grabowski_ab_2007}. It could be problematic in the case of Pb, as the phonon frequencies are already quite low and high-volume variations can easily lead to imaginary nonphysical frequencies. For this reason, in the present study, we have limited the calculation to the LDA XC. A detailed study on functional dependency would be worthwhile, but we note that the effect of SOC on phonon frequencies has been reported to be more important than the change in the XC functional and its corresponding lattice parameter~\cite{verstraete_density_2008}.

\Cref{subfig:band_structures_no_lattice_expansion,subfig:band_structures_dos_no_lattice_expansion} show the Fermi-level aligned band structure and DOS of \ce{Pb} with and without SOC using their respective optimized lattice spacing. \ce{Pb} having two bands crossing the Fermi level, the two resulting sheets in the Fermi Surface are denoted $\alpha$ and $\beta$, and are marked by arrows. Globally, SOC has little effect on the band structure and the DOS. The main differences can be seen in the band structure where the degeneracies are lifted close to the $\Gamma$ and $W$ points, which is consistent with what was previously reported in Refs.~\cite{heid_effect_2010,corso_ab_2008,verstraete_density_2008,horn_electronic_1984}. Notably, almost no changes occur around the Fermi level, which means that the Fermi surface is negligibly affected by SOC.%  apart from small variations of total surface area.

\Cref{subfig:phonon_dispersions_no_lattice_expansion} shows the phonon dispersion of Pb with and without SOC using their respective optimized lattice parameter. The two transverse modes $T_1$ and $T_2$, as well as the longitudinal mode $L$ are identified by arrows. As reported by others~\cite{ponce_epw:_2016,corso_ab_2008,heid_effect_2010,verstraete_density_2008}, taking into account SOC softens the phonon frequencies, such that agreement with the inelastic neutron scattering data from Ref.~\cite{brockhouse_crystal_1962} is improved. Globally, this softening occurs almost everywhere in the BZ and appears to be strongest near the $X$ point. %  point despite the small difference in the lattice parameters. 
Furthermore, SOC improves the agreement with the kinks in the dispersion attributed to Kohn anomalies~\cite{kohn_image_1959} on the $\Gamma-K$ line and close to the $L$ point. % Such anomalies were reported to be better described with a small enough electronic occupations smearing factor and high enough $\vk$ grid\cite{corso_ab_2008}.
% It was also noted in Refs. \cite{corso_ab_2008,verstraete_density_2008} that SOC combined with a small enough smearing factor were needed in order to correctly describe the Kohn anomaly seen in the experimental data on the $K-\Gamma$ line}. Using the DFT parameters listed in Sec. \ref{sec:computational_details}, it is noteworthy that we do not capture this feature as well as the previous studies since we used a relatively coarse $\vq$-point mesh. However, we infer that this anomaly have close to no effects on the phonon free energy and other phonon-dependant quantities as the error introduced by neglecting SOC across the whole BZ is much larger than the error caused by the anomaly itself.

==> sections/intro.tex <==
\section{Introduction}
\label{sec:intro}

% General intro on EPC ??
% The Electron-phonon interactions (EPI) are fundamental to many thermodynamical properties of materials, including the temperature dependence of transport properties\cite{giustino_electron-phonon_2017}, conventional superconductivity\cite{bardeen_theory_1957}, band structure renormalization\cite{allen_theory_1976} and Kohn effects\cite{kohn_image_1959}\todo{more effects?}.

% general intro on thermodynamic properties
% too general...
% The development of high-throughput and machine learning based methods in order to quickly and cheaply predict material properties within the design process of functional applications have seen a drastic rise in the past decade\cite{curtarolo_high-throughput_2013,bishara_state---art_2023,jain_commentary_2013_materials_project}. Indeed, exploring the vast material space through experimental trial and error is both expensive and time consuming. However, such techniques are usually based on databases of material properties computed from an \abinitio technique such as Density Functional Theory (DFT)\cite{hohenberg_inhomogeneous_1964,kohn_self-consistent_1965}. Therefore, the accuracy is mainly limited by the DFT results which are often considered state-of-the-art\cite{bishara_state---art_2023}. Nowadays, 

% general intro on Pb
The thermodynamic properties of bulk face center cubic (FCC) lead, Pb, have been studied in details over the past century. Indeed, as one of the simplest elemental metals with a single atom in its unit cell, Pb is a well-known conventional superconductor with one of the highest transition temperature and electron-phonon coupling (EPC) strength~\cite{schrieffer_effective_1963,scalapino_strong-coupling_1966,savrasov_electron-phonon_1996,de_gironcoli_lattice_1995,floris_two-band_2007}.

% paragraph on SOC
Furthermore, Pb exhibits strong spin-orbit coupling (SOC) effects in both its electronic and vibrational degrees of freedom~\cite{verstraete_density_2008,heid_effect_2010,corso_ab_2008,vosko_influence_1965,liu_linear-response_1996,smirnov_effect_2018,ponce_epw:_2016,sklyadneva_electron-phonon_2012}. As such, from the point of view of \abinitio calculations, Pb was a prime candidate to be studied within the framework of Density Functional Perturbation Theory (DFPT) in its early years~\cite{savrasov_electron-phonon_1996,de_gironcoli_lattice_1995,liu_linear-response_1996} and in the past decade when SOC was added to the DFPT frameworks~\cite{corso_ab_2008,verstraete_density_2008,heid_effect_2010,sklyadneva_electron-phonon_2012}. It was shown that SOC is needed to correctly describe the finer structures in the phonon dispersion, such as Kohn anomalies~\cite{corso_ab_2008,verstraete_density_2008,heid_effect_2010,sklyadneva_electron-phonon_2012,smirnov_effect_2018}, where a general phonon softening throughout the whole first Brillouin Zone, particularly pronounced at the $\vq=X$ point, was observed. The overall results agree better with inelastic neutron scattering data taken at \qty{100}{\kelvin} than with the results obtained without SOC~\cite{brockhouse_crystal_1962,brockhouse_old_1961}. Generally, SOC also changes the EPC matrix elements which induces striking changes in the Eliashberg spectral function and the electronic self-energy~\cite{heid_effect_2010,sklyadneva_electron-phonon_2012}.

% specific intro on the resistivity of Pb
Over the years, many thermodynamical properties of Pb have been computed from first principles, including free energy~\cite{grabowski_ab_2007,smirnov_effect_2018}, equation of states~\cite{strassle_equation_2014,smirnov_effect_2018}, phonon dispersion and EPC strength~\cite{savrasov_electron-phonon_1996,de_gironcoli_lattice_1995,liu_linear-response_1996,corso_ab_2008,heid_effect_2010,verstraete_density_2008,grabowski_ab_2007,ponce_epw:_2016,rittweger_phonon_2017,sklyadneva_electron-phonon_2012}, thermal expansion (TE)~\cite{grabowski_ab_2007} and transport properties~\cite{savrasov_electron-phonon_1996,ponce_epw:_2016,smirnov_effect_2018,rittweger_phonon_2017}. Regarding the latter, the published calculated phonon-limited temperature-dependent resistivity curves, albeit close to experiments, all present some discrepancies at high temperatures, which remains an open question.
% Samuel does not like the following so removed
%Likewise, for general phonon properties, most of the disagreements with respect to experimental data seen in the earlier work of \citet{savrasov_electron-phonon_1996} were accounted for by including SOC as shown by \citet{ponce_epw:_2016} and \citet{smirnov_effect_2018}. Because electron transport in Pb at high temperatures is mainly limited by the EPC, the remainder of this discrepancy has yet to be explained. At first glance, as the EPC depends on structural properties, one could argue that the TE of Pb could influence the resistivity at high temperatures and narrow the gap with experimental results.
Instead, for harmonic vibrational properties, most of the disagreements with respect to experimental data seen in the earlier work of \citet{savrasov_electron-phonon_1996} were accounted for by including SOC as shown by \citet{smirnov_effect_2018} and \citet{ponce_epw:_2016}.
% Hence, in this work, we focus on computing from first principles the phonon-limited temperature dependent resistivity of Pb while including both SOC and TE effects.
%Inspired by an earlier detailed analysis of the \abinitio carrier mobility in Silicon\cite{ponce_towards_2018}, we aim to explore possible solutions to this discrepancy.
% Furthermore, as \abinitio phonon-limited electronic transport calculations derived from the Boltzmann Transport Equation (BTE) have gained a lot of attention in recent years. Better approximations have emerged like the so-called Iterative BTE (IBTE)\cite{ponce_towards_2018,claes_assessing_2022,ponce_first-principles_2020} which, in principle
%A tentative explanation could lie in the formalism employed to compute the conductivity. 

Additionally, the reported \abinitio computations of lead's resistivity were all done within approximated solutions to the Boltzmann Transport Equation (BTE), namely the Lowest-Order Variational Approximation (LOVA)~\cite{allen_new_1978,ziman_electrons_1960} used in Refs.~\cite{savrasov_electron-phonon_1996,ponce_epw:_2016,smirnov_effect_2018} or the Momentum Relaxation Time Approximation (MRTA) and the constant Relaxation Time Approximation (cRTA) used in Ref.~\cite{rittweger_phonon_2017}. As all these methods are different approximations of a more general approach called Iterative BTE (IBTE)~\cite{ponce_first-principles_2020} and because a recent report showed significant differences between the IBTE, MRTA, and cRTA schemes~\cite{claes_assessing_2022}, we have yet to see if a higher level of theory could explain these discrepancies observed in Pb at high temperatures. 

In this work, we use Density Functional Theory (DFT) within the Quasi Harmonic Approximation (QHA) to compute the effect of TE and SOC on \ce{Pb}'s thermodynamical properties, namely the bulk modulus and its pressure derivative, the heat capacity and the phonon-limited temperature dependence of its electrical resistivity. The latter is computed using the state-of-the-art IBTE formalism which has not been applied to \ce{Pb} so far. Furthermore, to the author's knowledge, we first report the computation of \ce{Pb}'s TE, heat capacity, and bulk modulus pressure derivative with SOC. % effects included. Finally, we computed the effect of TE on Pb's resistivity both with and without SOC which, to our knowledge, has never been done before.
The theoretical framework is laid out in Sec.~\ref{sec:method} and the computational methodology in Sec.~\ref{sec:computational_details}. The results obtained are shown and discussed in Sec.~\ref{sec:results}. Finally, we present our conclusions and outlook.

% General intro + stating our goal
% In the past decade, there has been an increasing interest for first principles calculations of transport properties of materials limited by Electron-Phonon Interactions (EPI) by solving the linearized Boltzmann Transport Equation (BTE), in particular it's self-consistent or iterative form (IBTE)\cite{ponce_first-principles_2020,ziman_electrons_1960}. Indeed, finding solutions to the IBTE based on Density Functional Theory (DFT) calculations constitute a state-of-the art \abinitio approach to compute predictive values of carrier mobilities and conductivities \cite{ponce_first-principles_2020}, Hall mobilities and other transport phenomena involving electric and magnetic fields for both metals and semi-conductors\cite{macheda_magnetotransport_2018,macheda_theory_2020,ponce_drift_2022,ma_first-principles_2022}.

%Recent development enabled the computation of Hall mobilities and other transport phenomena involving magnetic fields\cite{macheda_magnetotransport_2018,macheda_theory_2020,ponce_drift_2022,ma_first-principles_2022}.

%Fully solving the IBTE from DFT calculation is challenging as one needs the phonon frequencies, the EPI matrix elements, the electronic dispersion and the electronic velocities accross the full Brillouin Zone (BZ) on very fine grid samplings\cite{li_electrical_2015,liu_first-principles_2017,ma_first-principles_2018,ponce_towards_2018}. % This is especially difficult for metals as the presence of a Fermi surface creates a discontinuity in the electronic occupations which makes the BZ energy integrals hard to converge. Luckily, this problem is typically alleviated by smoothing these occupations with a smearing function\todo{cite smearing litterature?}. However, despite 
% Additionnally, in metals, compared to the mainstream Ziman resistivity formula\cite{ziman_electrons_1960} and Allen's Lowest Order Variationnal Approximation (LOVA)\cite{allen_new_1978}, the IBTE scheme makes less assumptions on the shape of the Fermi surface and on the dispersions of the electron-phonon coupling properties\cite{ponce_first-principles_2020}. In any case, the equations involved to get the transport properties usually require very fine sampling of the Brillouin Zone (BZ) integrals and, thus, are challenging to converge\cite{li_electrical_2015,ponce_first-principles_2020,ponce_first-principles_2021_hall}\todo{probably we could cite a lot of paper for that}. 
% Luckily, progress have been made in recent years in order to use very efficient interpolation techniques developed for this purpose thus enabling such calculations in real materials. Examples include Maximally Localized Wannier Functions (MLWF)\cite{ponce_first-principles_2021_hall,ponce_drift_2022,ponce_hole_2019,ponce_route_2019,ponce_towards_2018,giustino_electron-phonon_2007}, coarse-grid padding for the electron-phonon coupling (EPC) matrix elements\cite{brunin_phonon-limited_2020}, Fourier interpolation for phonon frequencies\cite{baroni_phonons_2001,giannozzi_quantum_2020}, linear interpolation for EPI matrix elements\cite{li_electrical_2015}, etc. Hence, transport calculations employing the full IBTE scheme are now routinely produced with great accuracy with respect to experiments, \eg in Si\cite{li_electrical_2015,ma_first-principles_2018,fiorentini_thermoelectric_2016,ponce_towards_2018}, Diamond \cite{lofas_transport_2013,macheda_magnetotransport_2018}, GaAs\cite{liu_first-principles_2017,zhou_ab_2016,ma_first-principles_2018,lee_ab_2020}, GaN\cite{jhalani_ultrafast_2017,ponce_route_2019,ponce_hole_2019}, $\beta$-Ga\textsubscript{2}O\textsubscript{3}\cite{ghosh_ab_2016,kang_fundamental_2017}, halide perovskites\cite{ponce_origin_2019_perovskite}, Sr\textsubscript{2}RuO\textsubscript{4}\cite{abramovitch_combining_2023} and more \todo{talk about the rise of 2D materials?}. Additionally, a recent report showed significant differences between IBTE results and other approximated forms such as the Self Energy Relaxation Time Approximation (SERTA), the Momentum Relaxation Time Approximation (mRTA) and the constant Relaxation Time Approximation (cRTA)\cite{claes_assessing_2022}, thus advocating for the use of this technique instead of the other ones.

% However, despite these advances, few transport calculations involving the full IBTE formalism were reported in metals. Indeed, to our knowledge, IBTE results were only reported for Al\cite{li_electrical_2015} and, recently, for titanium carbide MXenes\cite{boussadoune_electronic_2023}. In this work, we apply this formalism in FCC Pb and we explore the effects of thermal lattice expansion (TE) and spin-orbit coupling (SOC) on the electrical resistivity.

% Specific intro on Pb
% In this work, we make use of the IBTE formalism in order to study the phonon limited resistivity of bulk FCC Pb from first principles. The transport properties of Pb using fully \abinitio calculations were already reported both using the Lowest Order Variationnal Approximation (LOVA) in Refs. \cite{savrasov_electron-phonon_1996,ponce_epw:_2016,smirnov_effect_2018} and using the SERTA and cRTA by Ref. \cite{rittweger_phonon_2017}. 

% It was already appearant from Refs. \cite{ponce_epw:_2016, smirnov_effect_2018} that Spin-Orbit Coupling (SOC) effects need to be taken into account in order to correctly describe lead's conductivity. Indeed, among all elemental crystals, Pb has one of the highest EPC strength yielding one of the highest superconducting critical temperature. This made Pb a principal case of study during the early days of the Eliashberg Theory of superconductivity\cite{heid_effect_2010,schrieffer_effective_1963,scalapino_strong-coupling_1966}. In addition to transport properties, It was shown that as well that one needs to consider SOC in order to correctly describe numerous properties such as the electronic degrees of freedom\cite{anderson_fermi_1965,verstraete_density_2008}, the unusually soft phonon dispersion uncluding the kinks due to Kohn anomalies\cite{heid_effect_2010,corso_ab_2008,de_gironcoli_lattice_1995} and the EPC matrix elements\cite{schrieffer_effective_1963,scalapino_strong-coupling_1966}. 

% Furthermore, the lattice parameter can also strongly influence the phonon properties of materials. As such, we also hypothesize that including TE will affect the conductivities, especially at high temperature where this effect is largest.
% pas sur de l'utilité de parler des autres formalismes si on ne les compare pas
% In the case of semiconductors, mobility calculations have now been routinely computed 
% Luckily, under some approximations, the IBTE can be simplified to give other formalisms which are easier to compute from a first principles point of view. Examples include the Self Energy Relaxation Time Approximtion (SERTA)\todo{cites}, the momentum Relaxation Time Approximation (mRTA)\cite{mustafa_ab_2016,ponce_first-principles_2020,ziman_electrons_1960} or its constant counterpart (cRTA)\cite{madsen_boltztrap2_2018,pizzi_boltzwann:_2014}.%, thus placing the IBTE scheme at a higher level of theory compared to these other approaches. 


% The main bottleneck of this approach is the Brillouin Zone $\vk$ and $\vq$ points sampling that require a very fine grid in order to account for the rapidly varying $\delta$ functions present in the formalism.
%Even though this approach yields predictive results for many materials, metals have seldom been studied using this approach. Indeed, the first fully \abinitio calculations on metals were done using Allen's LOVA approach by Savrasov \etal \cite{savrasov_electron-phonon_1996,savrasov_linear-response_1994}. Since then, 

%Indeed, most first principles calculations of metallic resistivities employed the Lowest Order Variational Approximation (LOVA) of the BTE. Since the LOVA approach uses approximations that discards variations of scattering rates across the Fermi surface\cite{ziman_electrons_1960,ponce_first-principles_2020,allen_new_1978}, it is thus limited to isotropic materials in principle. Furthermore, the LOVA formalism can be described as semi-empirical as it requires an arbitrary definition of the number of charge carriers participating to conduction\cite{ponce_first-principles_2020}, thus hindering real ab initio calculations. Nonetheless, LOVA have been successfully employed to predict the temperature-dependent resistivity of elemental metals\cite{savrasov_electron-phonon_1996,savrasov_linear-response_1994,bauer_electron-phonon_1998,pinski_calculated_1981}, alloys\cite{liu_direct_2015}, disordered metals\cite{liu_direct_2015} and even graphene\cite{park_electronphonon_2014}\todo{Cite more examples?}. Other examples: Sr\textsubscript{2}RuO\textsubscript{4}\cite{deng_transport_2016}.
%However, the transport properties of metals using fully ab initio methods based on the IBTE have seldom been reported.
% However, for metallic systems, published results are scarce and, to our knowledge, only the temperature-dependant resistivity of Al was reported with this scheme\cite{li_electrical_2015}. Nonetheless, other systems were also studied albeit under other approximated schemes like the mRTA, the Self-Energy Relaxation Time Approximation (SERTA) or the Lowest Order Variational Approximation (LOVA). LOVA results were obtained as early as the birthing days of DFPT by Savrasov \etal for several elemental metals\cite{savrasov_linear-response_1994,savrasov_electron-phonon_1996,bauer_electron-phonon_1998}. More recently, SERTA and mRTA results were obtained for Al\cite{jain_thermal_2016,li_electrical_2015}, Ag\cite{jain_thermal_2016,li_anomalously_2022}, Au\cite{jain_thermal_2016,li_anomalously_2022}, Cu\cite{li_anomalously_2022} and Pb\cite{rittweger_phonon_2017}. In all cases, results are in relatively good agreement with experiments.

% Hence, in this work, we aim to improve on the previously reported phonon-limited transport properties by computing fully \abinitio solutions to the self-consistent IBTE formalism in Pb while considering SOC and TE effects. 
%The authors claim that the reason why this is the case is because the integrand of the equations involved is proportional to the derivative of the Fermi-Dirac distribution which, they argue, is only relevent close to the Fermi level within several $k_BT$ where $k_B$ is the Boltzmann constant and $T$ the temperature\cite{rittweger_phonon_2017}. While this derivative is highest in this region, the range of integration gets larger at high temperature. Ou je m'en vas avec ça???
%or the Lowest Order Variationnal Approach (LOVA) in . In the latter, a detailed description of the phonon-scattering times across the Fermi surfaces have been reported. It was shown that, even for an isotropic material like Pb, there can be great variations in the strength of the scattering mechanism between different points in the BZ \todo{cite numerical results? / relevent to say this?}. However, their reported resistivities in Pb bears strong resemblance to the LOVA results by Savrasov \etal\cite{savrasov_linear-response_1994,} \todo{double check ref} which departs strongly from experimental results at high temperature which is shown in Fig. \todo{XX}.

%Pb is a metal with Face-Centered Cubic Bravais Lattice with only one atom in its unit cell. Among all elemental crystals, Pb has one of the highest electron-phonon coupling strength yielding one of the highest superconducting $T_c$ which made it a principal case of study during the early development of the Eliashberg theory of superconductivity\cite{heid_effect_2010,schrieffer_effective_1963,scalapino_strong-coupling_1966}. Its unusually soft phonon dispersion also present some wiggles and kinks due to Kohn anomalies\cite{corso_ab_2008,de_gironcoli_lattice_1995} which makes this material interesting from the point of view of \abinitio calculations. Recently, Rittweger \etal reported on the variations of the $\vk$-dependent structure of the Éliashberg function and various other electron-phonon related quantities accross the Fermi surfaces of Pb\cite{rittweger_phonon_2017}. Furthermore, they showed electronic transport computations using various approximation schemes including the relaxation time approximation (RTA)  

%One of the first fully ab initio DFT calculation of lead's resistivity was carried out by Savrasov~\etal where the LOVA approched was used\cite{savrasov_electron-phonon_1996}.  Despite showing good agreements for other elemental metals, their approach didn't yield accurate results for Pb. One explanation might lie in relativistic effects that were not taken into account. 
%Pb being a heavy element ($Z=82$), relativistic effects are important and need to be taken into account in order to get an accurate description of this material for both the electronic and atomic degrees of freedom\cite{vosko_influence_1965,corso_ab_2008,anderson_fermi_1965,verstraete_density_2008}.
%Furthermore, the LOVA approach by itself might not be adequate for Pb because one of its Fermi surface is heavily distorted\cite{bertoni_third_1974,anderson_fermi_1965}. Furthermore, Rittweger~\etal recently showed the highly anisotropic aspect of the lead's electron-phonon relaxation time across the Fermi surfaces\cite{rittweger_phonon_2017}. They also computed lead's resistivity with the IBTE formalism which yielded better agreements with experiments than the LOVA approach. However, discrepancy at high temperature is still found despite a higher level of theory. We note that they did not include SOC in their calculations and that they used the experimental lattice parameter of Pb \todo{make sure of this}. In this section, we explore the effects of SOC and lattice parameters on Pb's phonon-limited resistivity as computed from the IBTE formalism.
%Indeed, it has been shown that SOC effects are deemed important in order to get an accurate representation of the EPC matrix elements and phonon dispersions \cite{corso_ab_2008,heid_effect_2010}.
%In addition, the interatomic force constants rely on the lattice spacing \todo{need to cite something?}, thereby TLE might have a strong influence at high temperature \todo{maybe change this phrasing once final results are known}.\\

% Pb intro
% Pb is an archetypal elemental type I superconducting metal. However, it has proven elusive to accurately describe using



%In the early days of DFPT in the 1990s, the resistivity of simple elemental metals have been calculated from first principles using the Lowest Order Variational Approach (LOVA)\cite{savrasov_electron-phonon_1996,savrasov_linear-response_1994,bauer_electron-phonon_1998}. Albeit giving generally good results with respect to experimental data, this method is only valid for isotropic materials with spherical Fermi surfaces. Furthermore, it is intrinsically semi-empirical as it relies on a drude-like parameter specifying the number of carriers that participates to the conduction, thus hindering fully ab initio predictions\cite{ponce_first-principles_2020,ziman_electrons_1960}. More recent studies computed the effects of spin-orbit coupling (SOC) and disorder in magnetic metals and alloys using this method\cite{liu_direct_2015}. Jing et al. studied 2D metallic MXenes\cite{jing_electron-phonon_2020} using this technique.\todo{reformulate and cite more recent LOVA (and/or cRTA) metal papers}. In addition, the LOVA cannot be used to describe anisotropic materials and, to our knowledge, there are no reports of fully ab initio transport calculations on such materials. Rittweger et al. recently used the IBTE formalism to show that the phonon-limited scattering time is highly anisotropic in Pb\cite{rittweger_phonon_2017}. However, spin-orbit coupling effects were not included in the calculation whereas it was deemed important to get a accurate electron-phonon coupling (EPC) matrix elements \cite{heid_effect_2010,corso_ab_2008}.

%\textbf{Summary of what we did}\\
%In this work, we use the IBTE scheme in order to compute the conductivities of bulk Pb, Mg, Zn and Cd. We compare the addition of SOC and TLE and show that these are needed to increase the accuracy of the resistivity at high temperature.
%In the case of Pb, Rittweger et al. made a detailed investigation of the $\vk,n$-dependent electron-phonon relaxation time $\tau_{n\vk}$ and other EPC related quantities and explicitly showed their anisotropic character\cite{rittweger_phonon_2017}. Furthermore, the authors computed the phonon-limited conductivity going beyond the LOVA approximation. In the following, we improve on their work by exploring the effects of SOC which have been shown to be essential for a good description of the EPC matrix elements and of the phonon dispersion\cite{heid_effect_2010,corso_ab_2008}. In addition, we explore the effects of lattice thermal expansion as the lattice parameter strongly influences the interatomic force constants which, in turn, affects the EPC matrix elements\todo{ref needed?}. For the case of Mg, Zn and Cd which are all anisotropic materials with hexagonal crystal structures, we show that the IBTE formalism correctly describes the anisotropic nature of their conductivity tensors.


==> sections/lattice_expansion.tex <==
% merged with previous section
% \subsection{Volumetric Effects on Ground State Properties}
% \label{sec:volumetric_effects_on_gs}

% The temperature-dependent lattice parameter of Pb was computed by minimizing the Helmholtz free energy $F(V, T)$ of the system with respect to the unit cell volume $V$ at a given temperature $T$. In crystals, this free energy can be decomposed in an electronic $U(V)+F_{\text{el}}$ and phononic $F_{\text{ph}}$ terms yielding\cite{ponce_hole_2019,palumbo_lattice_2017,baroni_density-functional_2010}

% \begin{equation}
%     \label{eq:free_energy}
%     F(V,T)=U(V) + F_{\text{ph}}(V,T) + F_{\text{el}}(V,T),
% \end{equation}

% where $U(V)$ is the static clamped-ion energy at 0K and $F_{\text{el}}(V,T)$ is the free energy due to thermal electronic excitations.
% %In Eq. \eqref{eq:free_energy}, $F_{\text{el}}$ is the sum of the volume-dependent clamped-ion static energy at $T=0K$ and the energy due to electronic thermal excitations.
% Within the Quasi-harmonic approximation (QHA), the vibrational term can be written as\cite{palumbo_lattice_2017,ponce_hole_2019}

% \begin{align}
%     \label{eq:free_energy_phonons}
%     \begin{split}
%         F_{\text{ph}}(V,T)=&\frac{1}{2N_{\vq}}\sum_{\vq\nu}\bigg\{\hbar\omega_{\vq\nu}(V)\\
%         &+kT\ln\left.\left[1-\exp\left(-\frac{\hbar\omega_{\vq\nu}(V)}{kT}\right)\right]\right\},
%     \end{split}
% \end{align} 

% where $N_{\vq}$ is the number of $\vq$ points in the BZ and $\omega_{\vq\nu}(V)$ is the phonon frequency for branch $\nu$ and wavevector $\vq$ for a given primitive cell volume $V$.
For each volume listed in \cref{sec:computational_details}, we computed the ground state and phonon properties. The changes in the band structure and DOS of \ce{Pb} using these variations are depicted in \cref{subfig:band_structures_lattice_expansion_nosoc,subfig:band_structures_dos_lattice_expansion_nosoc} without SOC and \cref{subfig:band_structures_lattice_expansion_soc,subfig:band_structures_dos_lattice_expansion_soc} with SOC. The shaded areas represent the change of eigenvalues upon a change in volume with respect to the Fermi energy. %The red shared areas represent a compression and the blue shaded areas correspond to an expansion of the volume. 
We observe that volume variations do not drastically change the band structures and have little to no effect on the DOS at the Fermi level. In general, a higher volume (blue) decreases the bandwidths and vice versa for decreasing volume (red). From this we conclude that both SOC and lattice variations have negligible effect on the electronic structure close to the Fermi level.

The phonon dispersions are shown in \cref{subfig:phonon_dispersions_lattice_expansion_nosoc} without SOC and in \cref{subfig:phonon_dispersions_lattice_expansion_soc} with SOC. We see that the cell volume inversely correlates with the phonon frequencies, where smaller volumes yield higher frequencies, and vice versa. This is expected because a smaller volume generally gives higher interatomic force constants, which, in turn, increases the phonon frequencies. Hence, contrasting with the electronic band structure which is more sensitive to SOC than to the lattice parameter, the phonon dispersion is more sensitive to the volume than to SOC. The effect is so strong that the phonon softening induced by SOC at $X$ is enhanced to the point where the structure becomes unstable above an \qty{8}{\percent} dilation of the unit cell volume. This is seen in \cref{subfig:phonon_dispersions_lattice_expansion_soc} where the frequencies become imaginary in the vicinity of $\vq=X$. Still, \ce{Pb} is known to be stable up to a temperature of \qty{600}{\kelvin} where its experimental variation in the volume of the unit cell is close to \qty{8}{\percent} with respect to its low temperature value~\cite{grabowski_ab_2007}. Therefore, such imaginary frequencies as these volumes should not occur, and we infer that there are possible mechanisms beyond the QHA that might stabilize the system.\\

\subsection{Fermi Surface Nesting and Phonon Linewidths}
\label{sec:nesting}

\begin{figure}%
    \centering
    % \includegraphics{figures/nesting_function_with_sliders_v4.pdf}
    % all these subfloats are to create fake subfigures for cleveref
    \subfloat{\includegraphics{figures/nesting_function_with_sliders_v6.pdf}\label{subfig:nestings_zeta_nosoc}}% a
    \subfloat{\label{subfig:nestings_gzeta_nosoc}}%b
    \subfloat{\label{subfig:nestings_linewidth_nosoc}}%c
    \subfloat{\label{subfig:nestings_zeta_soc}}%d
    \subfloat{\label{subfig:nestings_gzeta_soc}}%e
    \subfloat{\label{subfig:nestings_linewidth_soc}}%f
    \caption{\label{fig:nestings}(a), (d) Electronic nesting function $\zeta_{\vq}$ from \cref{eq:nesting_function} where the dashed-dotted curve denote the contribution from intraband transitions within the $\alpha$ sheet, the dotted curve within the $\beta$ sheet and the dashed curves denote the interband transitions between the two. The plain curve is the sum of all the band-resolved nestings. (c), (f) Phonon linewidths $\gamma_{\vq\nu}$ computed from \cref{eq:phonon_linewidth} where the dashed-dotted and dashed curves represent contributions from the transverse modes $T_1$ and $T_2$ and the dotted curve represent the longitudinal mode $L$. The plain curves represent the sum of all linewidths. (b, e) $g$-weighted nesting function $\gamma_{\vq\nu}/\omega_{\vq\nu}$. Mode resolved contributions are depicted with the same line styles as for (c) and (f). (a-f) The  black lines are computed at the DFT-optimized volume $\Vdft$ while the blue shaded area spans the curves with increasing volumes up to $\delta V/\Vdft=\qty[retain-explicit-plus]{+6}{\percent}$ while the red shaded area represents decreasing volumes $\delta V/\Vdft=\qty{-6}{\percent}$. (d), (e) and (f) include SOC while (a), (b) and (c) do not. %Because the phonon frequencies become imaginary with SOC at a volume variation \qty[retain-explicit-plus]{\geq +8}{\percent}, we only show volumetric variations between \qtylist[retain-explicit-plus]{-6;+6}{\percent} in order to focus the discussion on physical behaviors.
    }
\end{figure}

To shed light on the SOC-induced phonon softening in Pb, we compute the Fermi surface nesting function using \cref{eq:nesting_function} with its band-resolved version $\zeta_{nm\vq}$. A detailed study of $\zeta_{nm\vq}$ without SOC was already reported by \citet{rittweger_phonon_2017} where it was shown that both interband and intraband transitions play an important role in the nesting. In this section, we expand this analysis with SOC, the EPC matrix elements and volume variations.

The nesting function is shown in \cref{subfig:nestings_zeta_nosoc,subfig:nestings_gzeta_soc} respectively without SOC and with SOC. As for \cref{fig:band_structures,fig:phonon_dispersions}, the shaded areas represent the regions spanned by the curves computed by expanding (blue) or compressing (red) the volume. We distinguish between the intraband nesting for the $\alpha$ sheet (dashed-dotted curve) and the $\beta$ sheet (dotted curve), the interband nesting between the two sheets (dashed curve) and the total sum of all of these (plain curve). We observe that the total nesting function increases with SOC by a factor of \qtyrange{5}{15}{\percent} depending on $\vq$. Furthermore, the nesting does indeed peak at $\vq =X$, which explains why the phonon softening at this point is higher. From the band resolved curves, we see that this peak is mainly due to interband nesting, whereas the intraband nesting is mostly constant across the Brillouin Zone except in the vicinity of $\Gamma$ where it diverges in an integrable way. Also, the intraband transitions are much larger with the $\beta$ sheet than for the $\alpha$ sheet, which is even lower than the interband nesting. This is interesting, as the shape of the $\beta$ sheet is quite complicated and anisotropic with its tubular geometry near the edge of the Brillouin Zone~\cite{rittweger_phonon_2017} compared to the $\alpha$ sheet, which holds seemingly large parallel surface areas~\cite{corso_ab_2008,rittweger_phonon_2017}. As such, intuitively, one could have expected that the nesting within the $\alpha$ sheet would be higher than within the $\beta$ sheet. Regardless, changing the volume has quantitative effects on the nesting where an increase in volume increases the nesting and vice versa. % Nevertheless, the change is similar with and without SOC, and all observations remain the same.
%
On the other hand, as mentioned in \cref{subsec:fs_nesting_ph_linewidth}, the nesting function only contains part of the information and one needs to take into account the EPC transition probabilities in order to analyze phonon softening. \Cref{subfig:nestings_linewidth_nosoc,subfig:nestings_linewidth_soc} show the mode-resolved phonon linewidth from \cref{eq:phonon_linewidth} (dashed, dashed-dotted and dotted curves) and their sum (plain lines) respectively, without SOC and with it. We observe that the total linewidth with SOC is much higher than without it, which implies that the phonon lifetimes are lower with SOC. % \todo{This weakens quasiparticle description? Does this imply further scattering and phonon softening?}
Also, we see that the phonon linewidth without SOC does not peak at $X$ compared to SOC, where it strongly peaks at this point. As such, we conclude that the EPC matrix element is enhanced at $X$ specifically with SOC. In particular, the peak at $X$ with SOC is due to the linewidth of the transverse modes $T_1$ (dashed-dotted curve) and $T_2$ (dashed curve) where a peak suddenly appears with SOC while the longitudinal mode $L$, which already peaks at $X$ without SOC, has its peak enhanced with SOC. Furthermore, there is a global trend upward throughout the Brillouin Zone of the linewidth for all modes, which correlates with the global phonon softening. As for the volumetric effect, it is almost non-existent for the linewidth which implies that the volume dependance of the EPC matrix elements is mostly contained within the phonon frequencies. Indeed, this is seen in \cref{subfig:nestings_gzeta_nosoc,subfig:nestings_gzeta_soc} where we show the phonon linewidth divided by their corresponding phonon frequencies, namely $\gamma_{\vq\nu}/\omega_{\vq\nu}$. This is equivalent to a nesting function weighted by the EPC matrix element, and doing so exposes the effect of the frequencies changes onto the matrix element as $g$ scales with $\omega_{\vq\nu}^{-1/2}$. Due to this relation and the fact that phonon frequencies strongly soften with SOC, the volume dependence of $\gamma_{\vq\nu}/\omega_{\vq\nu}$ increases with expanding volume with SOC (see the blue-shaded area in \cref{subfig:nestings_gzeta_soc}). Without SOC (\cref{subfig:nestings_gzeta_nosoc}), the volume dependence is much smaller and similar to the volume changes seen in the nesting function (\cref{subfig:nestings_zeta_nosoc}). As for the linewidth, the peak at $X$ remains with SOC while it is flattened without SOC.

In summary, electronic nesting does indeed peak at $X$, which is due to interband transitions (\cref{subfig:nestings_zeta_nosoc,subfig:nestings_zeta_soc}), and this is seen both with and without SOC. However, this nesting peak is flattened out by the EPC matrix element without SOC (\cref{subfig:nestings_gzeta_nosoc,subfig:nestings_linewidth_nosoc}), while it is enhanced with SOC (\cref{subfig:nestings_gzeta_soc,subfig:nestings_linewidth_soc}). This suggests that the softening of the phonon is stronger at $X$ because the EPC matrix element becomes larger. Simultaneously, the enhanced phonon softening with increasing volume affects only the frequency part of the EPC matrix element, which makes it even stronger. As such, we conclude that there is a mutual interplay between the phonon softening and the EPC matrix element, which yields the observed dispersion. Therefore, from our observations we conclude that not only nesting is important to explain the phonon softenings in Pb but also that the EPC matrix elements play a role in this phenomenon.

\subsection{Free Energy and thermal expansion}
\label{sec:free_energy}

% \begin{figure*}
%     \centering
%     \includegraphics[width=\linewidth]{figures/free_energy_figure.pdf}
%     \caption{(left) Phonon free energy in function of volume and temperature. $\times$ markers denote points where some phonon frequencies are imaginary. Dashed curves include SOC while plain ones do not. (middle) Electronic free energy in function of volume and temperature. The curves were shifted vertically such that the highest temperature at the equilibrium volume had a free energy equal to 0 without SOC and -20 meV with SOC such that the curves are visually distinguishable. The inset shows the variation of the free energy at each volume and temperature with respect to the free energy at $T=10K$. Dashed curves include SOC while the plain ones do not. (right) Ratio of the derivatives of the free energies of phonons and electrons at each temperature. The plain and (resp. dashed) curve denote an average over all volumes without SOC (resp. with SOC) while the blue (resp. orange) region delimit all computed values.}
%     \label{fig:free_energy_decomposition}
% \end{figure*}

\begin{figure}
    \centering
    \subfloat{\includegraphics{figures/free_energy.pdf}\label{subfig:free_energy_phonons}}% a
    \subfloat{\label{subfig:free_energy_electrons}}%b
    \subfloat{\label{subfig:free_energy_total}}
    \caption{\label{fig:free_energy}(a) $\Fph$ as a function of $\delta~V/\Vdft~\equiv~(V-\Vdft)/\Vdft$ and $T$. (b) $\Fel$ as a function of $\delta V/\Vdft$ and $T$. The curves were shifted vertically such that $F(\Vdft,T=\qty{610}{\kelvin})=0$ without SOC and \qty{-20}{\milli\electronvolt} with SOC. The inset shows $\delta~\Fel~=~\Fel(V, T)-\Fel(V,T=\qty{10}{\kelvin})$. (c) Total free energy $F=\Fel+\Fph$ as a function of $\delta V/\Vdft$ and $T$. The dashed (without SOC) and solid (with SOC) lines are fits to \cref{eq:birch-murnaghan}. The free energy is shifted vertically so that $F(\Vdft, T=\qty{10}{\kelvin})=0$. The black rounded (resp. squared) markers mark the position of $V_0(T)$ as extracted from the fit without SOC (resp. with SOC). (a)-(c) Dashed curves with square or $\times$ markers include SOC, while the plain ones with round markers do not. The $\times$ markers denote points where negative phonon frequencies occurred.
     % (right) Ratio of the derivatives of the free energies of phonons and electrons at each temperature. The plain and (resp. dashed) curve denote an average over all volumes without SOC (resp. with SOC) while the blue (resp. orange) region delimit all computed values.
    % (left) (right) Lattice parameter in function of temperature as computed by DFT within the QHA. We compare results which includes SOC (orange) or not (blue) against experimental measurements taken from \cite{feder_use_1958} (black stars). The inset shows the relative variation of the lattice parameter $\delta a / a_0 = (a - a_0)/a_0$ with respect to the lattice parameter $a_0$ obtained at $T=25\degree$.
    }
\end{figure}

From the volume-dependent phonon frequencies calculated, we use \cref{eq:free_energy_phonons} to obtain the phonon contribution to the free energy at various temperatures. The results are shown in \cref{subfig:free_energy_phonons} where the solid curves include SOC while the dashed ones do not. The $\times$ markers denote values where some phonon frequencies become imaginary. Such frequencies were simply discarded when using \cref{eq:free_energy_phonons}.% because their contribution was negligible when integrating over the whole BZ. This is due to the phase space around the imaginary frequencies, which is small compared to the rest of the BZ~\cite{grabowski_ab_2007}.
As expected, $\Fph$ decreases both if the temperature or volume increases. 

% (IN SUPLLEMENT MAYBE?) To make sure it was the case, we computed the contribution of the same modes at a lower stretching and we obtained less than 1\% of the total phonon free energy at the highest temperature. Therefore, we assessed that the points marked as $\times$ are still relevant for the determination of the temperature-dependant lattice parameter. For the electronic part of the free energy, usually the $F_{\text{el}}(V,T)$ term is neglected in insulators as the presence of a band gap makes it negligible at low temperature and $U(V)$ is taken as the total DFT energy at volume $V$. However, in metals, one cannot blindly discard this term as there is no electronic gap.

%  we can write $F_{\text{el}}(V,T)$ as\cite{mermin_thermal_1965}

% \begin{equation}
%     \label{eq:free_energy_electrons}
%     F_{\text{el}}(V,T)=U_{\text{el}}(V,T) - TS_{\text{el}}(T,V),
% \end{equation}

% where $U_{\text{el}}$ is the electronic internal energy at finite temperature for a unit cell volume $V$ and the entropy $S_{\text{el}}(T,V)$ is computed as

% \begin{equation}
%     \label{eq:entropy}
%     S_{\text{el}}(T,V) = -\sum_{i}f_i\ln f_i + (1-f_i)\ln(1-f_i),
% \end{equation}

%with $i$ being a composite index running over spins, $\vk$ and band while $f_i=f_i(T,V)$ is the occupation factor for an electron in state $\ket{i}$. Here, the temperature dependence of $f_i$ is carried explicitly by the chemical potential, but implicitly by the electronic eigenvalues which functionally depend on the electronic density which, itself, depends on the occupation factors. Therefore, $F_{\text{el}}$ needs to be computed self-consistently which can be done with Mermin's approach\cite{mermin_thermal_1965}. Typically, in non-metallic materials, the temperature dependence of $F_{\text{el}}$ can safely be ignored if the energy gap between the valence and conduction states is much larger than thermal energies\cite{ponce_hole_2019}. However, in metals, this is not the case and one cannot justify this approximation. Various methods exist in order to compute this temperature dependence and a previous work quantified the errors made by these different approaches in transition elements\cite{zhang_accurate_2017}. The most accurate one 

%For the electronic contribution to the free energy $U(V) + F_{\text{el}}(V, T)$, we employ the state-of-the-art approach introduced by Mermin\etal\cite{mermin_thermal_1965}, which was reported as the most accurate compared to other methods such as the DOS and the Sommerfeld approximations\cite{zhang_accurate_2017}. As such, for each sampled volume and temperature, we set  $U(V) + F_{\text{el}}(V, T)$ as the total energy of a full self-consistent field ground state DFT calculation where the single-particle occupation number are determined by a Fermi-Dirac distribution whose smearing is equal to the required physical temperature.
The electronic contribution to the free energy is shown in \cref{subfig:free_energy_electrons} for different temperatures and volumes. Again, the solid curves include SOC while the dashed ones do not. %All curves have been arbitrarily shifted vertically as described in the caption.
It is clear from this plot that most of the variation in the electronic free energy comes from changes in the lattice parameter. This is shown by subtracting the free energy at the lowest temperature for each curve: $\delta \Fel = \Fel(V, T) - \Fel(V, T=\qty{10}{\kelvin})$, as depicted in the inset. Doing so effectively cancels out the variation due to the lattice parameter, and the remainder only shows a temperature variation of less than \qty{2}{\milli\electronvolt}, which is roughly two orders of magnitude smaller than temperature variations in $\Fph$. As such, we conclude that, although \ce{Pb} is metallic, the term $\Felex$ is negligible compared to $\Fph$.

% This is shown on the rightmost panel of figure \ref{fig:free_energy_decomposition} where the ratio of the temperature gradient between the phonon and electron free energies is plotted. The curves denote the average over all volumes at a given temperature while the shaded area represents the span of all the ratios for all volumes. Orange data includes SOC while blue does not. This ratio is highest at low temperature denoting a stronger variation of the free energy of phonons versus temperature than the free energies of electrons at all volumes. From all this, it is possible to conclude that the phonon contribution to the free energies completely dominates the total free energy both in absolute value and in variation.

% Once the total free energy is known, we fit it at each sampled temperature with the third-order Birch-Murnaghan isothermal equation of state which can be written as\cite{birch_finite_1947,murnaghan_compressibility_1944}

% \begin{align}
%     \label{eq:birch-murnaghan}
%     \begin{split}
%         F(V, T) = E_0 +& \frac{9B_0V_0}{16}\left[\left(\frac{V_0}{V}\right)^{\frac{2}{3}}-1\right]^2\\
%         &\times\left\{\left[\left(\frac{V_0}{V}\right)^{\frac{2}{3}}-1\right]B_0' + \left[6-4\left(\frac{V_0}{V}\right)^{\frac{2}{3}}\right]\right\},
%     \end{split}
% \end{align}

% where $E_0$, $B_0$ and $B_0'$ are respectively the minimum of energy, the bulk modulus and the pressure-derivative of the bulk modulus at the equilibrium volume $V_0$. By extracting $V_0$ from the fit at each sampled temperature, we get the temperature-dependant lattice parameter $a(T)=\sqrt[3]{V_0(T)}$.
Finally, \cref{subfig:free_energy_total} shows the total free energy for different temperatures with respect to the sampled volumes. The solid and dashed curves are fits, respectively, to the third-order Birch-Murnaghan EOS (\cref{eq:birch-murnaghan}) with and without SOC. As for \cref{subfig:free_energy_phonons}, $\times$ markers denote points where negative phonon frequencies occurred. The black dots and squares denote, respectively, the $(V_0, F_0)$ pairs extracted from the fit for each temperature with and without SOC. % All curves are shifted vertically, as described in the caption.

% \subsection{Thermal Expansion}
% \label{sec:lattice_expansion}

\begin{figure}
    \centering
    \subfloat{\includegraphics{figures/lattice_expansion_plots.pdf}\label{subfig:lattice_expansion_absolute}}% a
    \subfloat{\label{subfig:lattice_expansion_relative}}%b
    \caption{\label{fig:lattice_expansion}
    % (a) Phonon free energy  $F_{\text{ph}}$ in function of volume and temperature. (b) Electronic free energy $F_{\text{el}}$ in function of volume and temperature. The curves were arbitrarily shifted vertically by a factor $F_0$ such that the highest temperature at the equilibrium volume had a free energy equal to 0 without SOC and -20 meV with SOC. The inset shows the variation of the free energy at each volume and temperature with respect to the free energy at $T=$10 K. (c) Total free energy in function of the volume and temperature. The plain (no SOC) and dashed (with SOC) lines are the third order Birch-Murnaghan equation of state fits (\cref{eq:birch-murnaghan}). The free energy is arbitrarily shifted  vertically such that the origin lies at the minimum of the free energy curve for $T=$ 10 K. The black rounded (resp. squared) markers marks the position of the $V_0$ as extracted from the Birch-Murnaghan fit without SOC (resp. with SOC).  (a)-(c) Dashed curves with square or $\times$ markers include SOC while the plain ones with round markers do not. The $\times$ markers mark points where negative phonon frequencies occurred.
     % (right) Ratio of the derivatives of the free energies of phonons and electrons at each temperature. The plain and (resp. dashed) curve denote an average over all volumes without SOC (resp. with SOC) while the blue (resp. orange) region delimit all computed values.
    (a) Lattice parameter as a function of temperature extracted from the free energy minimum $V_0$. (b) Lattice parameter relative variation $\delta a/a_0 = [a(T) - a_0]/a_0$ where $a_0$ is the lattice parameter at a reference temperature of $T=\qty{298}{\kelvin})$. Experimental data from Ref.~\cite{feder_use_1958} is shown as black stars. (a)-(b) The solid orange curve includes SOC, while the dashed blue one does not. DFT results without SOC using LDA (dashed red) and PBE (dashed yellow) from Ref.~\cite{grabowski_ab_2007} are shown for comparison.
    }
\end{figure}

\Cref{subfig:lattice_expansion_absolute} reports the values of the lattice parameter obtained from the EOS fits as a function of temperature. %The marker colors match the curve colors of the respective temperatures in \cref{subfig:free_energy_total}. Results with SOC are indicated with a dashed gray line with square markers, and without SOC with a solid gray line with round markers. 
For comparison, we show the DFT results without SOC obtained in Ref.~\cite{grabowski_ab_2007} in the figure with a red dashed line. %As their calculations did not include SOC, they match our solid curve.
Their LDA results matches ours without SOC closely. Further comparison is also possible with experimental measurements from Ref.~\cite{feder_use_1958} denoted by black stars. We observe that SOC induces a higher absolute variation in the lattice parameter than without SOC, which places the equilibrium lattice parameter in better agreement with the experimental measurements at high temperature. Nonetheless, equilibrium volumes both with and without SOC remain lower than the experimental data, which is consistent with the fact that LDA typically underestimates the lattice parameter. PBE results from Ref.~\cite{grabowski_ab_2007} are indicated with a yellow line; they overestimate the equilibrium lattice parameter for all temperatures as it is also expected for this functional. The relative temperature variation $\delta a/a_0=(a-a_0)/a_0$ is shown in \cref{subfig:lattice_expansion_relative} where $a_0=a(T=\qty{298}{\kelvin})$.
%the relative variation with respect to the lattice parameter at $T=\qty{298}{\kelvin}$.
Without SOC, we observe that the slope is smaller than the experimental variation, while with SOC it is larger. In comparison, the PBE variation (without SOC) is the best matched to experimental measurements for this variation. To our knowledge, there are no reports on the temperature variation of the equilibrium lattice parameter computed using PBE with SOC for \ce{Pb}.

\subsection{Heat Capacity and Bulk Modulus}
\label{subsec:results_heat_capacity}

\begin{figure}
    \centering
    \includegraphics{figures/heat_capacity.pdf}
    \caption{\label{fig:heat_capacity}Decomposition of the heat capacity of \ce{Pb} at constant pressure in function of temperature. The solid orange curves include SOC while the dashed blue ones do not. Square markers denote the total heat capacity at constant pressure as computed from \cref{eq:heat_capacity_constant_pressure}, triangles represent the contribution from $\CVph$ and diamonds show the contribution from the $\alpha^2BV_0T$ term. We compare with experimental data from Ref.~\cite{arblaster_thermodynamic_2012} shown as black stars and DFT results without SOC from Ref.~\cite{grabowski_ab_2007} computed using the LDA (red dashed curve) and the PBE (yellow dashed curve) XC functionals.}
\end{figure}

\Cref{fig:heat_capacity} shows the heat capacity as computed from \cref{eq:heat_capacity_constant_pressure} using the equilibrium lattice volume $V_0$ and the isothermal bulk modulus $B$ extracted from the EOS fits. The dashed blue curves denote our results without SOC, while the solid orange curves include it. The total heat capacity at constant pressure as computed from \cref{eq:heat_capacity_constant_pressure} is shown using square markers. We also show the different contributions to \cref{eq:heat_capacity_constant_pressure} where triangles represent the $\CVph$ term and diamonds denote the $\alpha^2 BV_0(T)T$ offset. We also compare the results with previous reported DFT results computed without SOC by \citet{grabowski_ab_2007} and experimental data from Ref.~\cite{arblaster_thermodynamic_2012}. Our results without SOC are in excellent agreement with experimental and reference DFT data, while results with SOC overestimate the experimental data at high temperature. This is surprising, as both the phonon dispersion and TE are in better agreement with SOC than without SOC. This difference is mainly imputable to the last term of the right-hand side of \cref{eq:heat_capacity_constant_pressure} where $\alpha$, $V_0$ and $B$ are all higher with SOC than without, while $\CVph$ is almost the same with and without SOC. Meanwhile, the $\CVel$ term (not shown) is less than \qty{1e-2}{\boltzmannconstant} at \qty{600}{\kelvin} both with and without SOC and is thus negligible. It is interesting to note that the reported PBE results without SOC display better agreement with experimental data than our LDA results with SOC.

% \subsection{Bulk Modulus}
% \label{sec:bulk_modulus}

\begin{figure}
    \subfloat{\includegraphics{figures/bulk_modulus.pdf}\label{subfig:bulk_modulus}}
    \subfloat{\label{subfig:bulk_modulus_derivative}}
    \caption{\label{fig:bulk_modulus}(a) Bulk modulus of \ce{Pb}. (b) The pressure derivative of the bulk modulus. (a)-(b) The dashed blue and solid orange lines are results from this work respectively without and with SOC. Round markers represent the isothermal bulk modulus $B$ (a) or its pressure derivative $B'$ (b) as extracted from the third order Birch-Murnaghan fit of the free energy from the left panel of \cref{fig:lattice_expansion}. Meanwhile, square markers denote the adiabatic bulk modulus $\BA$ (a) or its pressure derivative $\BAprime$ (b) computed from \cref{eq:theory_adiabatic_bulk_modulus,eq:theory_adiabatic_bulk_modulus_derivative,eq:theory_adiabatic_bulk_modulus_derivative_offset}. The dashed yellow and teal lines represent the isothermal bulk modulus computed using the PBESol functional from Ref.~\cite{smirnov_effect_2018}. Other LDA results computed at $T=\qty{0}{\kelvin}$ are from Refs.~\cite{grabowski_ab_2007} (green triangle) and~\cite{dal_corso_projector_2012} (pink open triangle without SOC and gray open diamond with SOC). Adiabatic experimental data are from Refs.~\cite{strassle_equation_2014} (purple stars), \cite{miller_pressure_1969} (red stars) and \cite{vold_elastic_1977} (brown stars).
    }
\end{figure}

\Cref{subfig:bulk_modulus,subfig:bulk_modulus_derivative} show the temperature dependence of the adiabatic and isothermal bulk modulus calculated using \cref{eq:theory_adiabatic_bulk_modulus,eq:theory_adiabatic_bulk_modulus_derivative,eq:theory_adiabatic_bulk_modulus_derivative_offset}. The orange curves with square markers include SOC, while the blue curves with rounded markers do not. Plain curves represent the adiabatic bulk modulus, whereas dashed ones represent the isothermal bulk modulus and the same goes for the bulk modulus pressure derivative. We compare our results with experimental data taken from Refs.~\cite{waldorf_low-temperature_1962,vold_elastic_1977,strassle_equation_2014} for $\BA$, from Refs.~\cite{strassle_equation_2014,miller_pressure_1969} for $\BAprime$ and to DFT calculations from Refs.~\cite{grabowski_ab_2007,dal_corso_projector_2012,smirnov_effect_2018}. To our knowledge, there are no reports of DFT calculations of the full temperature dependence of the adiabatic bulk modulus and its pressure derivative for \ce{Pb}. Our results with SOC are in good agreement with experimental data at low temperature both for $B$ and $\BA$ whereas, our results show that neglecting SOC yields an overestimated adiabatic and isothermal bulk modulus. Furthermore, our isothermal results with SOC are in good agreement with previous PBEsol results from \citet{smirnov_effect_2018}.  % , though our results without SOC are quite different where this a strong offset between the curves with and without SOC at high temperature.
The high-temperature discrepancy with SOC is probably due to the one seen in the heat capacity as $\BA$ is directly proportional to it, see \cref{eq:theory_adiabatic_bulk_modulus}. Compared to other $T=\qty{0}{\kelvin}$ LDA calculations, both of our low-temperature results for $\BA$ and $\BAprime$ agree well with the ones from~\cite{grabowski_ab_2007} while the difference is much larger for Ref.~\cite{dal_corso_projector_2012}, although the latter did not use a free energy description. In the end, for the phonon dispersion, SOC seems to soften both the isothermal and adiabatic bulk modulus.

As for the bulk modulus pressure derivative depicted in \cref{subfig:bulk_modulus_derivative}, we observe a strong deviation from the experimental measurements where our results for $B'$ decrease with temperature while the experiments show an increase. Although it has a different temperature trend from the experimental measurements, the overall quantity is positive for all temperatures, which means that an increase in pressure would lead to an increase of the bulk modulus. Our low temperature results are also in good agreement with the previous $T=\qty{0}{\kelvin}$ result from Ref.~\cite{grabowski_ab_2007} without SOC. We see that including SOC causes $B'$ to decrease faster with temperature than without it.

==> sections/results.tex <==
\section{Results and Discussion}
\label{sec:results}

\input{sections/ground_state_properties}
\input{sections/lattice_expansion}
\input{sections/transport}

==> sections/theory.tex <==
\section{Method}
\label{sec:method}

\subsection{Thermodynamic Properties}

The thermodynamic properties of Pb can be computed from the Helmholtz free energy $F(V, T)$ curves of the system where $V$ is the unit cell volume and $T$ the temperature. In a system comprised of non-interacting electrons and phonons, the free energy can be decomposed into electronic $F_{\text{el}}$ and phononic $F_{\text{ph}}$ terms, which yields~\cite{ponce_hole_2019,palumbo_lattice_2017,baroni_density-functional_2010}:

\begin{equation}
    \label{eq:free_energy}
    F(V,T)=\Fph(V,T) + \Fel(V,T),
\end{equation}
\noindent
where $\Fel$ can further be decomposed in two contributions: $\Fel(V, T) = U(V) + \Felex(V, T)$ where $U(V)$ is the clamped-ion energy at~\qty{0}{\kelvin} and $\Felex(V,T)$ is the free energy due to thermal electronic excitations~\cite{ponce_hole_2019}. The $\Felex(V,T)$ term is typically neglected in insulators when the electronic energy gap is much larger than thermal energies. In metals, $\Felex$ cannot be discarded and we rely on the finite-temperature formulation of DFT introduced by \citet{mermin_thermal_1965}, which was reported to be the most accurate method for computing $\Felex$ compared to other approximations such as the density of states (DOS) approach or the Sommerfeld approximation~\cite{zhang_accurate_2017}. As such, for each sampled unit cell volume and temperature, we set $F_{\text{el}}(V, T)$ as the total energy of a ground-state DFT calculation where the single-particle occupation numbers are determined by a Fermi-Dirac distribution.

The vibrational contribution to the Helmholtz free energy can be written within the QHA, as~\cite{palumbo_lattice_2017,ponce_hole_2019}:

\begin{align}
    \label{eq:free_energy_phonons}
    % \begin{split}
    %     F_{\text{ph}}(V,T)=&\frac{1}{2N_{\vq}}\sum_{\vq\nu}\bigg\{\hbar\omega_{\vq\nu}(V)\\
    %     &+kT\ln\left.\left[1-\exp\left(-\frac{\hbar\omega_{\vq\nu}(V)}{kT}\right)\right]\right\},
    % \end{split}
    \Fph = \frac{\kB T}{N_{q}}\sum_{\substack{\vq\nu\\\omega_{\vq\nu}(V)\neq 0}}\ln\left[2\sinh\left(\frac{\hbar\omega_{\vq\nu}(V)}{2\kB T}\right)\right],
\end{align} 
where $N_q$ is the number of $\vq$ points in the first Brillouin Zone, $\omega_{\vq\nu}(V)$ is the phonon frequency for branch $\nu$ and wavevector $\vq$ for a given unit cell volume $V$ and $\hbar$ and $\kB$ are respectively the reduced Planck's and Boltzmann's constants.

Once $F(V, T)$ is known for a given set of temperatures and volumes, we extract the various thermodynamical properties by fitting it to the third-order Birch-Murnaghan isothermal equation of state which can be written as~\cite{birch_finite_1947,murnaghan_compressibility_1944}

\begin{multline} \label{eq:birch-murnaghan}
        F(V, T) = F_0(T) + \frac{9 B(T) V_0(T)}{16}\left[\left(\frac{V_0(T)}{V}\right)^{\frac{2}{3}}-1\right]^2\\
        \times\left\{\left[\left(\frac{V_0(T)}{V}\right)^{\frac{2}{3}}-1\right]B' + \left[6-4\left(\frac{V_0(T)}{V}\right)^{\frac{2}{3}}\right]\right\},
\end{multline}
\noindent
where $F_0$, $V_0$, $B$ and $B'$ are, the minimum of the free energy, the equilibrium volume, the isothermal bulk modulus and the pressure derivative, respectively. By extracting $V_0(T)$ from the fit at each sampled temperature, we obtain the temperature-dependent lattice parameter $a(T)$. 

% \subsection{Heat Capacity}
% \label{subsec:theory_heat_capacity}

The heat capacity at constant volume can be derived from the free energy using $\CV=-T\left.\frac{\partial^2F}{\partial T^2}\right|_{\text{V}}$. As $F$ consists of a phonon term and an electronic term, we can also compute $\CV=\CVph + \CVel$ separately. For phonons, we have

\begin{equation}
    \label{eq:cv_phonons}
    \CVph(T) =\kB\sum_{\vq\nu}\left(\frac{\hbar\omega_{\vq\nu}}{2\kB T}\right)^2\sinh^{-2}\left(\frac{\hbar\omega_{\vq\nu}}{2\kB T}\right),
\end{equation}
while the electronic part $\CVel$ is computed using a finite difference formula and interpolated at the equilibrium volume $V_0$. Most experiment are instead made at constant pressure which can be obtained as~\cite{wallace_thermodynamics_1998}:

\begin{equation}
    \label{eq:heat_capacity_constant_pressure}
    \CP = \CV + \alpha^2BV_0(T)T,
\end{equation}
where $B$ is taken from the free energy fits of \cref{eq:birch-murnaghan} and $\alpha(T)=\frac{1}{V_0}\left.\frac{\partial V_0}{\partial T}\right|_\text{P}$ is the linear TE coefficient evaluated at constant pressure $P$.

% \subsection{Bulk Modulus}
% \label{subsec:theory_bulk_modulus}

\Cref{eq:birch-murnaghan} allows the computation of the isothermal bulk modulus and its pressure derivative. But, as for the heat capacity, what is typically measured experimentally is the adiabatic bulk modulus, $\BA$, and its pressure derivative, $\BAprime$. The relationships between $\BA$ and $B$ are~\cite{wallace_thermodynamics_1998}
\begin{align}
    \label{eq:theory_adiabatic_bulk_modulus}
    \BA =& B \frac{\CP}{\CV}\\
    \label{eq:theory_adiabatic_bulk_modulus_derivative}
    \BAprime =& \left(\frac{\BA}{B}\right)^2B' + \BA^2  \left.\frac{\partial\Delta k}{\partial P}\right|_T,
\end{align}
\noindent
where $\Delta k=1/B - 1/\BA$ and

\begin{multline} \label{eq:theory_adiabatic_bulk_modulus_derivative_offset}
        \left.\frac{\partial\Delta k}{\partial P}\right|_T = \Delta k\left\{\Delta k \left[1 +\frac{1}{\alpha^2} \left.\frac{\partial \alpha}{\partial T}\right|_{\text{P}}\right]\right.\\
        \left.+\frac{2}{\alpha B^2} \left.\frac{\partial B}{\partial T}\right|_{\text{P}}-\frac{1}{B}\right\}.
\end{multline}

\subsection{Electronic Transport}
\label{sec:theory_electronic_transport}

The phonon-limited DC conductivity can be obtained by solving the full IBTE as~\cite{ponce_first-principles_2020}%\cite{ponce_towards_2018,giustino_electron-phonon_2017}

\begin{equation}
    \label{eq:conductivity_tensor}
    \sigma_{\alpha\beta} = -\frac{e}{(2\pi)^3}\sum_n\int d^3\vk v_{n\vk,\alpha}\partial_{E_\beta}f_{n\vk},
\end{equation}
\noindent
where $e$ is the electron charge, $\partial_{E_\beta}f_{n\vk}$ is the derivative of the occupation factor for the electronic state $\ket{n\vk}$, where $n$ is the band index and $\vk$ the wavevector, with respect to the electric field $\vE$ and $v_{n\vk,\alpha}=\braket{n\vk|(i/\hbar)[\hat{H}, r_\alpha]|n\vk}$ is the diagonal element of the electronic band velocity operator for the state $\ket{n\vk}$ with $H$ being the Kohn-Sham Hamiltonian and $\vectorr$ being the position operator~\cite{starace_length_1971}. Considering the latter, in this work, we explicitly compute the commutator in order to correctly capture the effects of the non-local part of the potential~\cite{read_calculation_1991,ponce_epw:_2016,ismail-beigi_coupling_2001,pickard_nonlocal_2003,ponce_first-principles_2021_hall}. This is in contrast to the so-called \textit{ local approximation} which is often used in transport calculations where $v_{n\vk,\alpha}$ is approximated as the gradient of the electronic Kohn-Sham eigenvalues. Without external fields, the occupation factor $f_{n\vk}$ reduces to the Fermi-Dirac distribution denoted as $f_{n\vk}^0$. In \cref{eq:conductivity_tensor}, the integral is carried out over the first Brillouin-Zone, Greek indices denote Cartesian directions, and the temperature dependence is contained within the occupation factor term. The $\partial_{E_\beta}f_{n\vk}$ can be computed using the linearized BTE formalism where, in the context of EPC scattering without magnetic fields and temperature gradients, it can be computed iteratively from~\cite{ponce_towards_2018,ponce_first-principles_2020}

\begin{multline}\label{eq:ibte}
        \tau_{n\vk}^{-1}\partial_{E_\beta} f_{n\vk} = e\frac{\partial f_{n\vk}^0}{\partial\epsilon_{n\vk}}v_{n\vk,\beta}+\frac{2\pi}{\hbar}\sum_{m\nu}\int\frac{d^3\vq}{\Omega_{\text{BZ}}}|g_{mn\nu}(\vk,\vq)|^2\\
        \times[(1+n_{\vq\nu}-f^0_{n\vk})\delta(\Delta_{\vk,\vq}^{nm}+\hbar\omega_{\vq\nu})\\
 +(n_{\vq\nu}+f^0_{n\vk})\delta(\Delta_{\vk,\vq}^{nm}-\hbar\omega_{\vq\nu})]\partial_{E_\beta}f_{m\vk+\vq},  
\end{multline}
\noindent
where $\Omega_{\text{BZ}}$ is the Brillouin-Zone volume, $g_{mn\nu}(\vk,\vq)$ is the EPC matrix element which measures the coupling strength between states $\ket{n\vk}$ and $\ket{m\vk+\vq}$ via a phonon with a wavevector $\vq$ on branch index $\nu$, $n_{\vq\nu}$ is the Bose-Einstein occupation factor for that phonon mode and $\Delta_{\vk,\vq}^{nm}=\epsilon_{n\vk}-\epsilon_{m\vk+\vq}$ is the single-particle electron eigenvalue difference between the initial and scattered state which are obtained from DFT. The scattering rate $\tau_{n\vk}^{-1}$ is defined as

\begin{multline} \label{eq:relaxation_time}
        \tau_{n\vk}^{-1} = \frac{2\pi}{\hbar}\sum_{m\nu}\int\frac{d^3\vq}{\Omega_{\text{BZ}}}|g_{mn\nu}(\vk,\vq)|^2\\
        \times[(1-f^0_{m\vk+\vq}+n_{\vq\nu})\delta(\Delta_{\vk,\vq}^{nm}-\hbar\omega_{\vq\nu})\\
         +(f^0_{m\vk+\vq}+n_{\vq\nu})\delta(\Delta_{\vk,\vq}^{nm}+\hbar\omega_{\vq\nu})].
\end{multline}
\noindent
In \cref{eq:ibte,eq:relaxation_time}, the EPC matrix element is computed at the linear-response level using the perturbed Kohn-Sham $V$ as $\epcg~=~\braket{m\vk+\vq|\partial_{\vq\nu}V|n\vk}$~\cite{giustino_electron-phonon_2017}. This formalism is at a higher level of theory than the LOVA approach~\cite{ponce_first-principles_2020}. Thus, it should be more accurate as the latter may be derived by averaging out the relaxation times on the Fermi surface and assuming all electrons within the partially filled conduction band participate equally to the transport~\cite{ziman_electrons_1960,grimvall_electron-phonon_1981,allen_new_1978,ponce_first-principles_2020} which might be inaccurate for materials with complex anisotropic Fermi surfaces such as Pb.
% Although, the former argument can be a good approximations for some materials like the Alkali metals, this is generally not true especially for more complex Fermi surfaces like the ones from Pb. For the latter assumption, even though electrons that are further away from the Fermi level have a harder time to scatter into an unoccupied state than the ones close to it, it does not mean that \textit{all} electrons in the unfilled bands participate \textit{equally} to the conduction. One needs to take into account the occupation factor of the initial state and of the states in which the electron can scatter into. As such, this assumption can be classified as arbitrary as the final resistivity obtained via the LOVA approach can be scaled using an arbitrary number of carriers. This further justifies the use of the full IBTE scheme instead of the LOVA approach in order to compute metallic resistivities in order to compare the results directly with experiments.

\subsection{Fermi Surface Nesting and Phonon Linewidth}
\label{subsec:fs_nesting_ph_linewidth}

The inclusion of SOC in the phonon calculation of Pb leads to phonon softening due to an increased electronic nesting within the Fermi surface~\cite{verstraete_density_2008,ponce_epw:_2016,heid_effect_2010,corso_ab_2008}, which can be computed using

\begin{equation}
    \label{eq:nesting_function}
    \zeta_{\vq} = s\sum_{nm}\zeta_{nm\vq}\equiv \frac{s}{N_k}\sum_{nm\vk}\frac{1}{N_{\vk}}\delta(\epsilon_{n\vk}-\epsF)\delta(\epsilon_{m\vk+\vq}-\epsF),
\end{equation}
\noindent
where $\epsF$ is the Fermi energy, $N_{k}$ is the number of $\vk$-points in the Brillouin Zone and $s$ is a spin factor, which is equal to \num{4} without SOC and \num{1} with it. We also define the band-resolved Fermi surface nesting $\zeta_{nm\vq}$ where $n$ and $m$ are band indices. A drawback of the nesting function is that it does not take into account the EPC matrix elements. Indeed, the nesting function acts like a joint density of states, and in order to get a more accurate picture, one can compute the phonon linewidths which, at low temperature, can be approximated as~\cite{allen_neutron_1972,giustino_electron-phonon_2017}

\begin{multline} \label{eq:phonon_linewidth}
    \gamma_{\nu\vq}  = \frac{2\pi \omega_{\vq\nu}}{N_{k}}  \\
   \times \sum_{\vk mn} \left|g_{mn\nu}(\vk,\vq)\right|^2\delta(\epsilon_{n\vk}-\epsF)\delta(\epsilon_{m\vk+\vq}-\epsF).
\end{multline}

==> sections/transport.tex <==
\subsection{Charged Carrier Transport}
\label{sec:transport}

% We compute the EPI limited DC conductivity by solving the fully iterative BTE. In the BTE formalism, the DC conductivity tensor is given by\cite{ponce_towards_2018,ponce_first-principles_2020,giustino_electron-phonon_2017}

% \begin{equation}
%     \label{eq:conductivity_tensor}
%     \sigma_{\alpha\beta} = -(2\pi)^3e\sum_n\int_{\text{BZ}}d^3\vk v_{n\vk,\alpha}\partial_{E_\beta}f_{n\vk},
% \end{equation}

% where $e$ is the electron charge, $v_{n\vk,\alpha}$ is the electronic band velocity for state $\ket{n\vk}$ and $\partial_{E_\beta}f_{n\vk}$ is the derivative of the occupation factor for that state with respect to the electric field. Without external fields, the $f_{n\vk}$ reduces to the Fermi-Dirac distribution denoted as $f_{n\vk}^0$. In Eq. \eqref{eq:conductivity_tensor}, Greek indices denote cartesian directions and all temperature dependence is fully contained within the occupation factor term. Within the BTE formalism in the context of EPI scattering without magnetic fields and temperature gradients, the $\partial_{E_\beta}f_{n\vk}$ term can be computed using\cite{ponce_towards_2018,ponce_first-principles_2020}

% \begin{equation}
%     \label{eq:ibte}
%     \begin{split}
%         \partial_{E_\beta}f_{n\vk}=& e\frac{\partial f_{n\vk}^0}{\partial\epsilon_{n\vk}}v_{n\vk,\beta}\tau_{n\vk}+\frac{2\pi\tau_{n\vk}}{\hbar}\sum_{m\nu}\int_{\text{BZ}}\frac{d^3\vq}{\Omega_{\text{BZ}}}|g_{mn\nu}(\vk,\vq)|^2\\
%         &\times[(1+n_{\vq\nu}-f^0_{n\vk})\delta(\Delta_{\vk,\vq}^{nm}+\hbar\omega_{\vq\nu})\\
%         &+(n_{\vq\nu}+f^0_{n\vk})\delta(\Delta_{\vk,\vq}^{nm}-\hbar\omega_{\vq\nu})]\partial_{E_\beta}f_{m\vk+\vq},
%     \end{split}    
% \end{equation}

% where $g_{mn\nu}(\vk,\vq)$ is the EPI matrix element representing the probability amplitude for electrons to scatter from state $\ket{n\vq}$ to state $\ket{m\vk+\vq}$ via a phonon with waveveector $\vq$ on branch index $\nu$ with a frequency of $\omega_{\vq\nu}$, $n_{\vq\nu}$ is the Bose-Einstein distribution evaluated at $\omega_{\vq\nu}$, $\Delta_{\vk,\vq}^{nm}=\epsilon_{n\vk}-\epsilon_{m\vk+\vq}$ is the single-particle electron eigenvalue difference between the initial and scattered state and $\tau_{n\vk}$ is the relaxation time which is defined as

% \begin{equation}
%     \label{eq:relaxation_time}
%     \begin{split}
%         \frac{1}{\tau_{n\vk}} =& \frac{2\pi}{\hbar}\sum_{m\nu}\int_{\text{BZ}}\frac{d^3\vq}{\Omega_{\text{BZ}}}|g_{mn\nu}(\vk,\vq)|^2\\
%         &\times[(1-f^0_{m\vk+\vq}+n_{\vq\nu})\delta(\Delta_{\vk,\vq}^{nm}-\hbar\omega_{\vq\nu})\\
%         &+(f^0_{m\vk+\vq}+n_{\vq\nu})\delta(\Delta_{\vk,\vq}^{nm}+\hbar\omega_{\vq\nu})].
%     \end{split}
% \end{equation}

\begin{figure}
    \centering
    % \includesvg[width=\linewidth]{figures/ibte_expansion_vs_no_expansion}
    \subfloat{\includegraphics{figures/transport_with_te_sliders.pdf}\label{subfig:transport_no_te}}
    \subfloat{\label{subfig:transport_with_te}}
    \caption{\label{fig:transport_results}(a) IBTE results without TE. The solid orange curves include SOC while the dashed blue ones do not. The dashed blue and solid orange curves with square markers were computed using the optimized geometry $\Vdft$ while the ones with round markers were computed using the experimental lattice parameter at room temperature of $a=\qty{4.95}{\angstrom}$ taken from Ref.~\cite{zagorac_recent_2019}. The purple, pink, gray and brown stars represent the experimentally measured resistivity from Refs.~\cite{hellwege_electrical_1982,moore_absolute_1973,cook_thermal_1974,leadbetter_energy_1966}. The green dashed curve is the resistivity obtained using the LOVA approach as reported in Ref.~\cite{savrasov_electron-phonon_1996} while the red dashed line represent MRTA results obtained with the experimental lattice parameter as reported in Ref.~\cite{rittweger_phonon_2017}. Both the green and red dashed curve neglects SOC. (b) Same as (a) except TE is included in the computation of the solid orange and dashed blue curves. The curves with squared markers make use of the TE computed from the minimum of the free energy $V_0(T)$ while the ones with round markers used the experimental lattice parameters taken from Ref.~\cite{feder_use_1958}.
    }
\end{figure}

In this section, we report our results for the phonon-limited temperature-dependent resistivity of Pb as computed using \cref{eq:conductivity_tensor,eq:ibte,eq:relaxation_time}. The results are shown in \cref{subfig:transport_no_te} without TE and in \cref{subfig:transport_with_te} with it. When TE is included, we compute a resistivity of $\rho=\qty{13.2}{\micro\ohm\centi\meter}$ without SOC and $\rho=\qty{28.2}{\micro\ohm\centi\meter}$ with SOC at $T=\qty{310}{\kelvin}$. When neglecting TE, we obtain $\rho=\qty{11.3}{\micro\ohm\centi\meter}$ without SOC and $\rho=\qty{21.9}{\micro\ohm\centi\meter}$. The experimental value at this temperature is approximately $\rho=\qty{22.2}{\micro\ohm\centi\meter}$~\cite{moore_absolute_1973}.
%
For comparison, we also show earlier results by \citet{savrasov_electron-phonon_1996} (green dashed curve) and \citet{rittweger_phonon_2017} (red dashed curve with rounded markers), where the former used Allen's formula~\cite{allen_new_1978} and the latter used the so-called Momentum Relaxation Time Approximation (MRTA)~\cite{ponce_first-principles_2020,claes_assessing_2022} without SOC. In MRTA, the second term of \cref{eq:ibte} is neglected and a geometric factor of $\left(1-\frac{\vv_{n\vk}\cdot\vv_{m\vk+\vq}}{|\vv_{n\vk}|^2}\right)$ is inserted within the integral of \cref{eq:relaxation_time}. For both the red and green dashed lines, SOC was neglected. We compare against the experimental data from Refs.~\cite{hellwege_electrical_1982,leadbetter_energy_1966,cook_thermal_1974,moore_absolute_1973} which are represented by the purple, pink, gray and brown stars. For both panels, solid orange curves include SOC, whereas the dashed blue ones do not. Curves with square markers were computed using DFT geometry obtained from relaxation for \cref{subfig:transport_no_te} or from minimization of the free energy at each temperature, as shown in \cref{subfig:transport_with_te}. In contrast, the curves with round markers were computed using the experimental lattice parameter at room temperature taken from Ref.~\cite{zagorac_recent_2019} in \cref{subfig:transport_no_te} and the experimental temperature-dependent lattice parameters of Ref.~\cite{feder_use_1958} in \cref{subfig:transport_with_te}. We observe that curves computed using the experimental lattice parameter (curves with round markers) all have higher resistivity than their corresponding DFT analogs. This is expected as the experimental volume is higher for all temperatures, yielding softer phonons and increased EPC matrix elements. As such, this increases the probability that an electron diffuses via a phonon, thus decreasing the mean free path of electrons, which increases the resistivity. The same can be said when SOC is turned on (solid orange curves), where, in all cases, the resistivity increases. This was also seen using the LOVA approach, as reported in Refs.~\cite{ponce_epw:_2016,smirnov_effect_2018}. This is also consistent with the strong phonon softening seen with SOC, which increases the EPC matrix element, as discussed in \cref{subsec:fs_nesting_ph_linewidth}.

Focusing on \cref{subfig:transport_no_te}, the resistivity results obtained are all linear at high temperature. This is expected as the occupation number of phonons $n_{\vq\nu}\propto T$ when $kT\gg \hbar\omega_{\vq\nu}$ in \cref{eq:ibte,eq:relaxation_time}. We see that, as for the LOVA approach~\cite{ponce_epw:_2016,smirnov_effect_2018}, SOC needs to be taken into account to have values close to the experimental data. Nevertheless, this is still insufficient to explain the small deviation from linearity at high temperature, and thus we conclude that the IBTE is unable to explain the discrepancy seen in previous reports. When introducing TE, we see that DFT results without SOC do indeed get a small non-linear component at high temperature but, with SOC, this effect is much stronger which makes the resistivity increase rapidly at high temperature.

In addition, the IBTE formalism gives a slightly different result than the so-called Self-Energy Relaxation Time Approximation (SERTA) approach where the second term on the right hand side of \cref{eq:ibte} is neglected. At $T=\qty{310}{\kelvin}$, the SERTA overestimates the resistivity with TE by \qty{14.7}{\percent} without SOC and by \qty{5.7}{\percent} with SOC compared to the IBTE. Without TE, the relative difference is similar where the SERTA overestimates the resistivity by \qty{16.1}{\percent} without SOC and \qty{7.0}{\percent} with SOC compared to the IBTE. See the Supporting Information for a comparison of the SERTA and IBTE at all temperatures~\cite{Goudreault2024_SI}.

% we see a global linear trend of the resistivity in function of the temperature (left panel). This is expected for metals with a phonon-dominant scattering process like in Pb\todo{cites; talk about Motte-Ioffe-Regel limit? Drude formula?}. As such, the solution of the BTE when considering only electron-phonon interactions is consistent with this trend except at high temperature where there is a small deviation from linearity. We hypothesize that this deviation is partly due to the thermal expansion of the lattice which is discussed further below.

\begin{figure}
    \centering
    \subfloat{\includegraphics[width=1.0\columnwidth]{figures/relaxation_times_figure_v4.pdf}\label{subfig:relaxation_times_no_te_nosoc}}
    \subfloat{\label{subfig:relaxation_times_no_te_soc}}
    \subfloat{\label{subfig:relaxation_times_te_nosoc}}
    \subfloat{\label{subfig:relaxation_times_te_soc}}
    % \vskip-0.5cm  % this works but not vspace?
    % see https://tex.stackexchange.com/questions/686212/vspace-number-cm-between-subfigure-and-subcaption-works-in-back-directi
    \caption{\label{fig:relaxation_times}EPC relaxation times inverse as computed from \cref{eq:relaxation_time} in function of the difference between the corresponding single-particle energy eigenvalues $\epsilon_{n\vk}$ and the chemical potential $\mu$. (b) and (d) include SOC while (a) and (c) do not. (c) and  (d) include TE while (a) and (b) do not. It is worth noting here that $\mu$ is temperature-dependant.}
\end{figure}

To shed light on the anomalously high resistivity with SOC and TE, in \cref{fig:relaxation_times} we show the inverse relaxation times resolved by temperature computed from \cref{eq:relaxation_time} as a function of their corresponding electronic eigenvalue $\epsilon_{n\vk}$. The results without SOC are shown in \cref{subfig:relaxation_times_no_te_nosoc,subfig:relaxation_times_te_nosoc}, while those with SOC are shown in \cref{subfig:relaxation_times_no_te_soc,subfig:relaxation_times_te_soc}. Meanwhile, the results without TE are depicted \cref{subfig:relaxation_times_no_te_nosoc,subfig:relaxation_times_no_te_soc} and those with TE are shown on \cref{subfig:relaxation_times_te_nosoc,subfig:relaxation_times_te_soc}.
%
%In all cases, the relaxation times seem to be grouped into three distinct groups. But since the derivative of the occupation functions $\partial f^0_{n\vk}/\partial \epsilon_{n\vk}$, which multiplies $\tau_{n\vk}$ in \cref{eq:ibte}, is only significant in a region centered on the chemical potential whose width is roughly equal to the temperature, the central group closest to the chemical potential is the only one contributing to the transport physics.
%
In all cases, increasing the temperature decreases the relaxation times, which in turn increases the resistivity. This is due to the increased phonon population, as described in the previous paragraph. When SOC is turned on, we see that the inverse relaxation time increases by about \qty{\sim 25}{\percent} before TE is considered. Interestingly, the trend is reversed for the upper group, even though it does not affect the resistivity, while the lower one is unaffected by SOC. The effect of TE without SOC has a similar effect to that of SOC and increases the inverse relaxation times by \qty{\sim 10}{\percent}. However, the effect of TE with SOC is more drastic as it yields an increase of \qty{\sim 75}{\percent}, thus tripling the effect of SOC alone. This signals an interplay between SOC and TE with respect to relaxation times, and these behaviors are correlated with those seen in $\gamma_{\vq\nu}/\omega_{\vq\nu}$ depicted in \cref{subfig:nestings_gzeta_soc}. Indeed, the phonon linewidth is increased by SOC but is independent of the volume, while the phonon frequencies are sensitive to it. As such, EPC matrix elements experience a strong increase with volume because the phonon dispersion is significantly softened by the increase in volume (see \cref{subfig:phonon_dispersions_lattice_expansion_soc}). Therefore, we conclude that the anomalously high resistivity with TE and SOC is caused in part by the strong phonon softening and by the high TE with SOC as shown in \cref{subfig:lattice_expansion_absolute}. We postulate that a better description of the TE with SOC might significantly change the computed resistivity at high temperature.

% Fig. \ref{fig:relaxation_times} show the inverse of relaxation times  in function of the corresponding single-particle energy eigenvalues. The left panel includes SOC effects while the right one does not. The insets represents the relaxation times without taking into account the thermal expansion of the lattice that is, the temperature effects only come from the change in electronic occupations and the chemical potential. Unsurprisingly, increasing the temperature decreases the relaxation times as the fermi-dirac distribution $f^0_{m\vk+\vq}$ for states whose energies are close to the chemical potential is roughly proportional to the temperature, while the Bose-Einstein distribution converges to a constant at high temperature. Concerning SOC effects, we see that SOC considerably decreases the lifetime. This is expected as SOC enables scattering between states of different spins which increases the number of states an electron can diffuse into, thus decreasing the relaxation time. Furthermore, the effects of thermal lattice expansion seems to further decrease the relaxation times but only when SOC is turned on. This is unexpected as one could infer that changing the lattice parameter would affect the relaxation times in a similar manner whether or not SOC is included.\todo{Probably need more explanations here / physical interpretation}

% In all cases, SOC introduces a global increase in resistivity across the whole temperature range. This is \todo{(mainly?)} due to the decrease in relaxation times with SOC as discussed in the previous paragraph. When neglecting the thermal expansion of the lattice and using the optimized geometry as computed with DFT and including SOC effects we get the resistivity in closest agreement with the experimental data (dashed blue curve on the left panel of Fig. \ref{fig:transport_results}). Meanwhile, using the experimental lattice parameters increases drastically the resistivity both with and without SOC (orange curves). This is expected since the LDA underestimates the lattice parameter compared to the experimental value and increasing it generally weakens the electron-phonon coupling\todo{?}

%A steady-state electrical current can flow through a material by applying a static external electric field $\vE$. Following Ohm's law, the current density, $\vJ$, created by this driving field is linearly proportional to the latter where the proportionality constant is the so-called conductivity tensor $J_\alpha=\sigma_{\alpha\beta}E_\beta$, where Greek indices denote cartesian directions and repeated indices are summed over. Within the BTE framework, the current density can be written as $J_\alpha=-(2\pi)^3e\sum_n\int_{\text{BZ}}d^3\vk f_{n\vk}v_{n\vk,\alpha}$, where $e$ is the electron charge,  $f_{n\vk}$ is the perturbed occupation factor which reduces to the Fermi-Dirac distribution in absence of electric fields\cite{ponce_towards_2018} and $v_{n\vk,\alpha}$ is the electronic velocity in the direction of the current. From Ohm's law, $\sigma_{\alpha\beta}$ can be computed by deriving $J_\alpha$ with respect to the field $E_\beta$ which yields\cite{ponce_towards_2018,ponce_first-principles_2020,giustino_electron-phonon_2017}
